Structural results for the Tree Builder Random Walk

We study the Tree Builder Random Walk: a randomly growing tree, built by a walker as she is walking around the tree. Namely, at each time $n$, she adds a leaf to her current vertex with probability $p_n \asymp n^{-\gamma}$, $\gamma\in (2/3,1]$, then moves to a uniform random neighbor on the possibly modified tree. We show that the tree process at its growth times, after a random finite number of steps, can be coupled to be identical to the Barab\'asi-Albert preferential attachment tree model. Thus, our TBRW-model is a local dynamics giving rise to the BA-model. The coupling also implies that many properties known for the BA-model, such as diameter and degree distribution, can be directly transferred to our TBRW-model, extending previous results.

==> A_k.fixed.tex <==
The purpose of this section is to demonstrate that when there are infinitely many growth times (i.e. $p_n$ is not summable),
and there are sufficiently many edges  grown at those times, the walk is never recurrent, and under a mild condition on $p_n$ (ruling out that the walk ``gets stuck'') it is transient.

Let $Z_n=w_n$ with probability $p_n$ and $Z_n=0$ otherwise. Here $\{w_n\}_{n\ge 1}$ is a non-decreasing numerical sequence such that $w_n\in \mathbb N\setminus \{0\}$.

We will denote  $\mathfrak P_n:=\sum_{k=1}^n p_k$,  
and for a sequence $\{a_n\}_{n\geq 1}$, we will write $\Delta a_i:=a_i-a_{i-1}$.
The graph distance between the root $o$ and vertex $v$ will be denoted by $d(o,v)$.
Finally, denote 
$\tau_n := \inf \Lbrace n > \tau_{n-1} \, : \, Z_n >0 \Rbrace\;$, with $\tau_0 \equiv 0$, and  $r_{i,j}:=\Pd_{T_0,o; \mathcal{L}}(\tau_i>j),i,j\in \mathbb N$;  note that $r_{i,j}$ is a function of the sequence  $\{p_n\}_{n\geq 1}$ only. 
\begin{remark}[Poisson-Binomial]
The $r_{i,j}$ can be computed for a fixed sequence of $p_n$'s using the identities of the Poisson-Binomial distribution, since the number of growths up to time $m$ follows a Poisson-Binomial distribution with parameters $m,p_1,...,p_m$ and mean $\mathfrak P_m$, for $m\ge 1$.
If this number is $K^{m,p_1,...,p_{m}}$ then 
$$r_{i,j}=P(K^{j,p_1,...,p_{j}}\le i-1)\;.$$
Since we only need an upper bound in the next result, we can simply use Chebyshev.  Indeed, if $Y_i:= \mathbb{1}\{Z_i >0\}$, i.e.,  the indicator of the $i$-th growth then $r_{i,j}= P(Y_1+...+Y_j\le i-1)$, and by the Chebyshev inequality,
\begin{equation}\label{Ch.bound}
  r_{i,j}\le  \frac{\sum_{k=1}^j p_k(1-p_{k})}{\left(\mathfrak P_j-i+1\right)^2}\le 
\frac{\mathfrak P_j}{\left(\mathfrak P_j-i+1\right)^2}\;,
\end{equation}
 provided $\mathfrak P_j>i-1.\hfill\diamond$
\end{remark}
\begin{theorem}[Transience]\label{thm:tr}
Assume that 
$\sum\limits_{n\ge 1}p_n=\infty$ to rule out obvious recurrence, and that there exists a numerical sequence $0<a_1<a_2,\dots$ such that
\begin{enumerate}
    \item $$\sum_{i=1}^{\infty}r_{i,a_{i}}<\infty;$$
\item $$\sum_{i=1}^{\infty}\frac{\Delta a_i}{w_{i-1}+1}<\infty.$$
\noindent Then the $\mathcal{L}$-\name is not recurrent.

If furthermore we assume that
\item \begin{equation}\label{mild.condition}
\sum_{n\ge 1} \min\{p_n,p_{n+1}\}=\infty.
\end{equation}
\end{enumerate}
then the $\mathcal{L}$-\name is transient: $\Pd_{T_0,o; \mathcal{L}}\left(\lim\limits_{n\to \infty} d(o,X_n)=\infty\right)=1$.
\end{theorem}
\begin{corollary}
For every non-summable sequence $\{p_n\}_{n\geq 1}$ there exists some sequence $\{w_n\}_{n\geq 1}$, making the \name{}  non-recurrent, and under Condition 3 of Theorem \ref{thm:tr} even transient.
\end{corollary}
\begin{example}[Transience]
Let $p_i:=\frac{1}{i+1}$, hence $\mathfrak P_n=\mathcal{O}(\log n)$. Then for any $\{w_i\}$ growing so fast that with some $\epsilon>0$
$$\sum_{i=1}^{\infty}\frac{2^{i^{1+\epsilon}}}{w_{i-1}+1}<\infty\;,$$
holds,
the $\mathcal{L}$-\name is transient. To verify this, pick $a_i:=2^{i^{1+\epsilon}},\ \epsilon>0.$ Then
by \eqref{Ch.bound}, $$r_{i,a_i}\le \frac{\mathfrak P_{a_{i}}}{(\mathfrak P_{a_{i}}-i+1)^2}\;,$$
which is $\mathcal{O}(i^{-1-\epsilon}),$ thus summable.$\hfill\diamond$
\end{example}
The next example shows that the condition \eqref{mild.condition} is indeed essential for transience.
\begin{example}[The walk is not recurrent and the walker is ``stuck'']
Consider the sequence of $p_n$'s $$1/2,1/2,1/3,1/4,1/4,1/8,1/5,1/16,...$$
which is obtained by ``combing'' the harmonic series $1/2,1/3,1/4,...$ and the convergent series 
$1/2,1/4,1/8,...$ together; condition \eqref{mild.condition} is not satisfied in this case.
A close look at the proof of Theorem \ref{thm:tr} reveals that for this choice of $p_n$ and sufficiently large $w_n$ (so that the first two conditions of Theorem \ref{thm:tr} are met) with positive probability $d(o,X_n)$ can be stuck between two positive integers forever.$\hfill\diamond$
\end{example}
\begin{proof}[Proof of Theorem \ref{thm:tr}]
We prove the result in three steps.

\medskip
\underline{STEP 1:} We now assume that \eqref{mild.condition} holds. Recall that $\tau_i$ is the $i$-th time of growth, $i\ge 1,$ 
and for $k\ge 1$, let
$$v_k:=\text{\ the ``father vertex'' launching $w_k$ new edges at}\ \tau_k;$$
$$A_k:=\{\exists i\ge 1: d(o, X_n)> d(o, v_k) \; \forall n\geq \tau_k +i\}\;.$$
Note the following. Writing simply $d(v)$ instead of $d(o,v)$, on the event $\limsup_k A_k,$ the walker
$X$ eventually leaves all closed (!) balls of radius $d(v_k)$ around $o$. In particular then, $d(v_{k+1})>d(v_k)$. Hence, in fact $X$ eventually leaves arbitrarily large closed balls, and this implies transience.
So, if we show that 
\begin{equation}\label{limsup=1}
    \Pd_{T_0,o; \mathcal{L}}\left(\limsup_{k\to\infty} A_k\right)=1\;,
\end{equation} then transience follows.

We start by showing that for any $\epsilon>0$ there is a deterministic integer $k_0=k_0(\epsilon)\ge 1$  such that if $k\ge k_0$ then  
\begin{align}\label{close.to.1}
\pi_k:=&P(A_k)\ge 1-\epsilon\;.
\end{align}
To achieve this,  first note that
\begin{equation}\label{union.bound}
\Pd_{T_0,o; \mathcal{L}}(\cap_{i=k}^{\infty}\{\tau_i\le a_i\})= 1-\Pd_{T_0,o; \mathcal{L}}(\cup_{i=k}^{\infty}\{\tau_i>a_i\})\ge 1-\sum_{i=k}^{\infty}r_{i,a_{i}}\;.
\end{equation}


\underline{Heuristic explanation for estimating $\pi_k$ from below:}
First note that clearly, $\tau_k\ge k$, thus $w_{\tau_k}\ge w_k$, given our monotonicity assumption on the $w_i$'s.
Consider the following strategy.
For each $k\ge 0$, on the time interval $[\tau_k,\tau_{k+1}-1]$ the walker chooses to increase her distance from $o$ every time she is at a vertex of degree $1+w_k$ or larger; each time this happens with probability  at least $w_k/(w_k+1)$.

We now claim that this strategy guarantees that $A_k$ occurs almost surely, that is, that the walker, while implementing this strategy, eventually leaves the ball of radius $d(v_k)$, whatever $k\ge 1$ is.

Indeed, for any $k\ge 1$, the event $v_k=v_{k+1}=v_{k+2}=...$ has probability zero. To see this recall \eqref{mild.condition} and note that at least one time out of any two consecutive times, the walker is at a vertex different from $v_k$. 
This means that the walker eventually stays at a distance from the origin which is not just at least $d(v_k)$ but also at least $d(v_{k+i})>d(v_k)$, with some $i\ge 1$. 

Since the above strategy guarantees that $A_k$ occurs a.s., by \eqref{union.bound} one has that
\begin{equation}\label{lower.bd.pik}
   \pi_k\ge \left(1-\sum_{i=k}^{\infty} r_{i,a_i}\right)\cdot\prod_{i=k}^{\infty}\left( \frac{w_{i-1}}{w_{i-1}+1}\right)^{\Delta a_i}, \quad k\ge 1\;.
\end{equation}


Using that for some $c>e$, 
$$\left( \frac{w_{i-1}}{w_{i-1}+1}\right)^{\Delta a_i}> c^{- \frac{\Delta a_{i}}{w_{i-1}+1}},\qquad i\ge 2,$$
it follows that
\begin{equation}\label{sum.product}\prod_{i=k}^{\infty}\left( \frac{w_{i-1}}{w_{i-1}+1}\right)^{\Delta a_i}\ge
\prod_{i=k}^{\infty}c^{- \frac{\Delta a_{i}}{w_{i-1}+1}}=c^{-\sum_{i=k}^{\infty} \frac{\Delta a_{i}}{w_{i-1}+1}}\;.
\end{equation}
Exploiting \eqref{lower.bd.pik} and \eqref{sum.product}  the bound $\pi_k>1-\epsilon$ follows if, with some appropriately small $\delta(\epsilon)>0$,
\begin{equation*}
\sum_{i=k}^{\infty} r_{i,a_i}<\delta(\epsilon)\text{\qquad and\qquad}
\sum_{i=k}^{\infty}\frac{\Delta a_i}{w_{i-1}+1}<\delta(\epsilon)\;,
\end{equation*}
which, in turn, are guaranteed for large enough $k$'s by our summability assumptions.

\medskip
\underline{STEP 2:}
So far, we have shown that, assuming  \eqref{mild.condition},  for some (deterministic) integer $k_0(\epsilon)\ge 1$,
$$\Pd_{T_0,o; \mathcal{L}}(A_k)\ge 1-\epsilon,\qquad \forall k\ge k_0(\epsilon).$$
By the reverse Fatou inequality then, $$\Pd_{T_0,o; \mathcal{L}}\left(\limsup_{k\to\infty} A_k\right)=\Pd_{T_0,o; \mathcal{L}}\left(\limsup_{i\to\infty} A_{k_{0}+i}\right)\ge 1-\epsilon.$$
Since $\epsilon>0$ was arbitrary, \eqref{limsup=1} follows, and hence we are done with showing transience under conditions 1-3.

\medskip
\underline{STEP 3:} To complete the proof of the theorem, a careful look at the first two steps reveals that if we drop \eqref{mild.condition}, then although the argument for the walker going out to infinity breaks down, it still follows that she will be bounded away from the root a.s., hence the process is not recurrent.
\end{proof}


==> Comments.on.speed.tex <==
These are some comments on speed -- note for ourselves only.

The following inequalities are meant in a very loose sense, between orders of magnitudes of random variables.

Since there has been many versions of the (attempted) transience proof, I just sketch here a simple argument
to be self contained.

Assume $p_n\searrow$, and note that out of every two consecutive times, at least one time is spent on a non-leaf. At those times at least with probabilities $p_2,p_2,p_4,p_4,...,$ we are on a non-leaf and an edge is grown. Let  

Let $d_n:=d(o,X_n)$ and let $\ell_n$ denote the time spent on leaves.
Let $$P^{even}_n:=p_2+p_4+...+
p_{\lceil n/2\rceil}.$$


Note that $P_n$ is on the same order as $P^{even}_n$ (up to a factor 2.)
\begin{itemize}
    \item When on a vertex of degree at least three, the drift is $1/3$, and this itself would give \emph{at least} a contribution $(1/3)P^{even}_n$, which is on the order $P_n$.
    
    \item The degree 2 vertices only introduce a fluctuation according to LIL, and the assumption is that this is smaller order. This is satisfied e.g. for the gamma case when $\gamma<1/2$.
    
    \item Finally, there are the degree one vertices (leaves) to handle. They decrease the distance $d_n$ by $\ell_n$.
\end{itemize}



So, using a very crude way of recording this,

$$P^{even}_n/3-\ell_n\le d_n.$$
On the other hand 
$$d_n\le P_n.$$
Here we ignore the lower order terms coming from the LIL, (so e.g. $\Theta(P_n)$ should be $\Theta(\sqrt{P_n\log\log P_n})$) but they do not change much the arguments.

Transience means $d_n\to\infty$. So any $P^{even}_n=P_n/3-\gamma_n$ works, where $\gamma_n\to\infty$.

Now, it may be that $\gamma_n=o(P_n)$, in which case all we know is that $\gamma_n\le d_n$. So in this case $d_n$ is not necessarily on the ``maximal'' order $\Theta(P_n)$, and $\ell_n$ is not on the order of $n$, only $\Theta(P_n)$.

==> degreedist.tex <==
%TEX root = main.tex

In this section, we prove  that the degree distribution of the random tree sequence $\{T_n\}_{n\geq 0}$ in the $\mathcal{L}$-\name with $L_n=\mathsf{Ber}(p_n)$, $p_n=\Theta(n^{-\gamma})$ and $\gamma \in (2/3,1]$ \comj{$\gamma \in (1/2,1]$} converges to a power-law distribution with exponent $3$, the very same limiting distribution as in the  Barabási-Albert model of \emph{preferential attachment} (PA) \cite{barabasi1999emergence,bollobas2001degree}. 

It will be useful to look at the random tree sequence~$\{T_n\}_{n\geq 0}$ only at the random times when the \name adds new vertices to the tree. For this reason, we begin by recursively defining the following sequence of stopping times:
\begin{equation}\label{def:tau}
\tau_k := \inf \Lbrace n > \tau_{k-1} \, : \, Z_n = 1\Rbrace\;,
\end{equation}
where $\tau_0 \equiv 0 $. In words, $\tau_k$ is the time when the $k$-th (new) vertex is added. 

It will be useful to understand the asymptotic behavior of the stopping times $\{\tau_k \}_{k\ge 0}$. \com{Let us begin  noticing that for $\gamma>1$,  $\tau_k=+\infty$, for all sufficiently large $k$, $\Pd_{T_0,x;\mathcal{L}}$-a.s.}. The following lemma, whose proof will be postponed to the end of this section, essentially tells us that in the regime $\gamma > 2/3$ \comj{$\gamma>1/2$}, we need to wait large amounts of time to see the walker adding another leaf.
\begin{lemma}[Growth times are rare]\label{lemma:limtauk} Consider a $\mathcal{L}$-\name, where $L_n = \mathsf{Ber}(p_n)$ with $p_n=\Theta(n^{-\gamma})$ and  $\gamma>2/3$. Then, there exists a sufficiently small $\delta > 0$, depending only on $\gamma$,  such that
	\begin{equation}\label{eq:tau-lemma}
	\lim_{k \rightarrow \infty} k^{2+\delta}\tau_{k}^{-\gamma} = 0\;, \quad  \Pd_{T_0,x; \mathcal{L}}\text{-a.s.}\;
	\end{equation}
\end{lemma}
\com{
\begin{lemma}[Growth times are rare]\label{lemma:limtauk} Consider a $\mathcal{L}$-\name, where $L_n = \mathsf{Ber}(p_n)$ with $p_n=\Theta(n^{-\gamma})$ and  $\gamma \in (0,1)$. Then, for all $\varepsilon< \frac{ 1}{(1-\gamma)}$ it holds that 	\begin{equation}\label{eq:tau-lemma2a}
	\lim_{k \rightarrow \infty} k^{\gamma\left(\frac{1}{1-\gamma} - \varepsilon\right)}\tau_{k}^{-\gamma} = 0\;, \quad  \Pd_{T_0,x; \mathcal{L}}\text{-a.s.}\;
	\end{equation}
\end{lemma}
%
\begin{remark}
Note that for $\gamma \in (1/2,1)$ (equivalently, $\frac{\gamma}{1-\gamma}>1$) by choosing $\varepsilon$ sufficiently small, the above lemma tells us that  there exists a sufficiently small $\delta > 0$, depending only on $\gamma$,  such that 	\begin{equation}\label{eq:tau-lemma2}
	\lim_{k \rightarrow \infty} k^{1+\delta}\tau_{k}^{-\gamma} = 0\;, \quad  \Pd_{T_0,x; \mathcal{L}}\text{-a.s.}\;.
	\end{equation}
\end{remark}
}
\comj{The new lemma is weaker beyond $2/3$. The reason is that we should  state what we actually proved. Namely, let ``wfmeas'' abbreviate ``with finitely many exceptions almost surely.'' Then 
\begin{enumerate}
    \item for any $\gamma\in (0,1)$ and $c<c_{\gamma}:=\frac{1}{1-\gamma}$, one has $$\tau_k\ge k^c,\ \text{wfmeas}.$$
    \item consequently,  for any $\gamma\in (0,1)$ and $\delta<\frac{\gamma}{1-\gamma},$ one has $$\lim_k \frac{k^{1+\delta}}{\tau_k^{\gamma}}=0,$$
    but it is \emph {better} to write this as follows: for any $\epsilon>0,$
    $$\lim_k \frac{k^{\gamma c_{\gamma}-\epsilon}}{\tau_k^{\gamma}}=0,$$
\end{enumerate}
and this is true for ANY $\gamma\in(0,1).$ (In particular, for $\gamma>1/2$ we have $\gamma c_{\gamma}>1.)$
}

For the rest of this proof fix $\delta>0$ such that \eqref{eq:tau-lemma} holds.
\begin{definition}[Good and bad time intervals]
With Lemma \ref{lemma:limtauk} in mind, we say that $\Delta \tau_k := \tau_k - \tau_{k-1}$ is \emph{good} if 
\begin{equation}\label{def:goodtau}
\Delta \tau_k \ge k^{2+\delta} +1\;,
\end{equation}
% for a fixed $\delta$ that will be chosen properly later.  
 and we say that it is \emph{bad} otherwise.
\end{definition}

\com{
\begin{definition}[Good and bad time intervals]
With Lemma \ref{lemma:limtauk} in mind (i.e., with the corresponding  $\delta$), we say that $\Delta \tau_k := \tau_k - \tau_{k-1}$ is \emph{good} if 
\begin{equation}\label{def:goodtau}
\Delta \tau_k \ge k^{1+\delta/2}\cdot {\rm diam}(T_{\tau_{k-1}}) +1\;,
\end{equation}
% for a fixed $\delta$ that will be chosen properly later.  
 and we say that it is \emph{bad} otherwise.
\end{definition}
}\comj{B/c of the above we can replace $k^{1+\delta/2}\cdot {\rm diam}(T_{\tau_{k-1}}) +1$ as follows. Pick $c_{\gamma}^*\in (2,c_{\gamma})$. Then the replacement is $k^{c_{\gamma}^{*}}\cdot {\rm diam}(T_{\tau_{k-1}}) +1$
}

To avoid clutter,   we will write $\widetilde{T}_k := T_{\tau_k}$, and $\widetilde{\vertexset{}}_k$ for the set of vertices of $\widetilde{T}_k$ and $\widetilde{\mathcal{F}}_k$ for $\mathcal{F}_{\tau_{k}}$. Notice that for any~$n \in (\tau_{k-1}, \tau_{k})$, $T_n$ and $\widetilde{T}_{k-1}$ has the same degree distribution. For this reason we focus our attention on the process $\{\widetilde{T}_k\}_k$.

Let us begin looking at the  evolution of the random graph model   $\{\widetilde{T}_k\}_k$ from a slightly different, although equivalent, perspective.   At any ``time'' step $k$, a new vertex $v_k$ and two half-edges,  $h_{k,1}$ and $h_{k,2}$,  are added to $\widetilde{T}_{k-1}$. The two half-edges account for the edge which connects the vertex $v_k$ to the tree $\widetilde{T}_{k-1}$. While the half-edge $h_{k,1}$  is always incident to the new vertex $v_k$, the half-edge $h_{k,2}$ will be attached  to the vertex in $\widetilde{\vertexset{}}_{k-1}$ where the random walk resides at time $\tau_k-1$, thus determining to which of the existing vertices the new vertex $v_k$ will be connected to in $\widetilde{T}_k$.
%

Leveraging on the above-mentioned   equivalent perspective of the evolution of $\{\widetilde{T}_k\}_k$,  we are going to introduce  a color-assignment process for  the half-edges which will be instrumental for proving the result. 
%
Specifically, at any time $k$, we color the two half-edges $h_{k,1}$ and $h_{k,2}$ in either \emph{blue} or \emph{red} according to the following rule: Let $B_{k-1}$ and $R_{k-1}$ denote the total number of half-edges blue and red  in $\widetilde{T}_{k-1}$, respectively (w.l.o.g, we assume $B_1=2, R_1=0$, which means that $T_0$ is a single edge whose half-edges are both blue). Then, for $k\ge 2$,
\begin{itemize}
	\item if $\Delta \tau_{k}$ is \textit{bad}, we color both $h_{k,1}$ and $h_{k,2}$ \textit{red};
	\item if $\Delta \tau_{k}$  is \textit{good}, we color $h_{k,1}$ \textit{blue}, while we flip a biased coin to decide the color of  $h_{k,2}$. The probability that $h_{k,2}$ is \textit{blue} is $B_{k-1}/2(k-1)$,  and 
	\textit{red} otherwise.
\end{itemize}
%
% \begin{enumerate}
% 	\item we choose a half-edge $h$ proportional to its random weight $\widetilde{w}_{k-1}(h)$ in $\widetilde{T}_{k-1}$ and duplicate it, creating $h_{k,1}$;
% 	\item  we add a new vertex $v_k$ together with a half-edge $h_{k,2}$ attached to it;
% 	\item we glue together the new half-edges to obtain the tree $\widetilde{T}_k$.
% \end{enumerate}
% Additionally, each half-edge in our trees is going to be painted \textit{red} or \textit{blue} according to some rules which we describe below.
% \begin{itemize}
% 	\item if $\Delta \tau_{k}$ is \textit{bad} we paint $h_{k,1}$ and $h_{k,2}$ \textit{red};
% 	\item if $\Delta \tau_{k}$ is \textit{good} we paint $h_{k,2}$ \textit{blue};
% 	\item the duplicate procedure preserves the color of an half-edge;
% \end{itemize}
Note that $B_{k-1}/2(k-1)$ is the ratio of blue half-edges in $\widetilde{T}_{k-1}.$
Note also that the color assignment depends on the evolution of $\{\widetilde{T}_k\}_k$ through the conditions $\Delta\tau_{k}$ being bad or good, which in turns depends on $\gamma$ (see, Equation~\eqref{def:goodtau}), but it does not depend on the position of the random walk at time $\tau_k-1$. 




As we shall soon show, in order to prove Theorem~\ref{thm:powerlaw}, it suffices to show that the empirical \emph{blue} degree distribution of $\widetilde{T}_k$  converges to~$4/d(d+1)(d+2)$. 
%
The first ingredient is to  show that the total number of \emph{red} half-edges is small compared to the total number of \emph{blue} half-edges. This is addressed in the next lemma, whose proof is deferred to the end of this section. 
%and $\mathbf{B}_k$ be the \textit{total number of vertices having at least one half-edge attached to it}.
\begin{lemma}[Not many red edges]\label{lemma:Rk} There exist $\varepsilon,\delta'>0$ depending on $\gamma$ only, such that for $k$ sufficiently large
\begin{equation*}
	\Pd_{T_0,x;\mathcal{L}} \left( R_k > k^{1-\varepsilon} \right) \le e^{-k^{\delta'}}.
	\end{equation*}
\end{lemma}
Next, we introduce some notation which will be instrumental in proving Theorem~\ref{thm:powerlaw}. Let $b_k(v)$ (resp. $r_k(v)$) be the \textit{blue} (resp. \textit{red}) degree of a vertex~$v$ in $\widetilde{\vertexset{}}_k$, that is, $b_k(v)$ (resp.  $r_k(v)$) counts  the number of blue (resp. red) half-edges incident to $v$ in $\widetilde{T}_k$. Also, for a fixed $d\in \mathbb{N}\setminus \{0\}$, let~$B_k(d)$ denote the number of vertices in $\widetilde{T}_k$ whose blue degree is exactly $d$, i.e.,
\begin{equation*}
B_k(d) := \sum_{v\in \widetilde{\vertexset{}}_k}\mathbb{1}\{b_k(v) = d\}\;.
\end{equation*}
Moreover, we say that a vertex $v \in \widetilde{\vertexset{}}_k$ is \textit{blue} if all half-edges incident to it are \textit{blue}.

\medskip 
Our main argument will rely on  stochastic approximation techniques \cite{robbins1951stochastic, benaim1999dynamics} to deal with the error arising from the fact that 
the blue degree of a vertex does not evolve according to a ``pure'' linear preferential attachment scheme, i.e., the probability of a vertex increasing its blue degree by one  is not simply proportional to its blue degree, but there is an (additive) error which must be controlled. 
%
To keep the paper self-contained, we state below the specific stochastic approximation framework  we shall use, which is taken \textit{ad litteram} from \cite{dereich2014robust}. 

\begin{lemma}[Stoch. Approx.; Lemma~3.1 in  \cite{dereich2014robust}]\label{lem:approximation}
	Let $\{Q_n\}_{n\geq 0}$ be a non-negative stochastic process satisfying the following recursion:
	\[
	Q_{n} - Q_{n-1} = \frac{1}{n} \left( \Psi_{n-1} -Q_{n-1} \Phi_{n-1} \right) +  M_{n}- M_{n-1}\;,
	\]
	where, $\{\Psi_{n}\}_{n\geq 0}, \{\Phi_{n}\}_{n\geq 0}$ are almost-surely convergent processes with deterministic limits $\psi>0$ and $\phi>0$, respectively, and $\{M_{n}\}_{n\geq 0}$ is an almost-surely convergent process. Then, $\lim_{n \to \infty}Q_n= \psi/\phi$, almost surely.
\end{lemma}
Together with the stochastic approximation framework, we will need a lemma which formalizes the discussion made in the previous paragraph. Roughly speaking, it says that whenever $\Delta \tau_k$ is good, the position of $X_{\tau_k -1}$ is selected according to a mixture of a preferential attachment scheme and some random error. 

%In order to simplify our notation, we will write $\widetilde{\theta}_k := \theta_{\tau_k}$ and $Z\circ \widetilde{\theta}_k$ to mean the process $\{Z_n\}_{n \ge 0}$ shifted by $\widetilde{\theta}_k$. \comj{Instead I introduced   the shifted sequence of laws at the beginning. So this should be deleted.}
\begin{lemma}[Almost PA at good times]\label{lemma:xtaucond} There exists $\delta>0$ such that for every $k\in \mathbb{N}$ and $t>k^{2+\delta}$, 
    \begin{align*}
	&\Pd_{ T_{\tau_{k-1}}, X_{\tau_{k-1}}; \mathcal{L}^{(\tau_{k-1})}}\left( X_{\tau_1 -1 } = v\mid \tau_1 = t\right)\\
	&\qquad\qquad= \frac{\degree{\tau_{k-1}}{v}}{2(k-1)} +\mathsf{error}(v,k)\;, \text{for}\  v\in \widetilde{T}_{k-1}\;,
	\end{align*}
	where the term $\mathsf{error}(v,k)$ represents a $\mathcal{F}_{\tau_{k-1}}$-measurable  random variable bounded by $e^{-k^\delta}, \Pd_{T_0,x;\mathcal{L}}$-almost surely. 
\end{lemma}
\com{
\begin{lemma}[Almost PA at good times]\label{lemma:xtaucond} For every $k\in \mathbb{N}$, every $\delta>0$ and $t>k^{1+\delta} {\rm diam}(T_{\tau_{k-1}})$,
    \begin{align*}
	&\Pd_{ T_{\tau_{k-1}}, X_{\tau_{k-1}}; \mathcal{L}^{(\tau_{k-1})}}\left( X_{\tau_1 -1 } = v\mid \tau_1 = t\right)= \frac{\degree{\tau_{k-1}}{v}}{2(k-1)} +\mathsf{error}(v,k)\;,\quad \text{for}\  v\in {T}_{\tau_{k-1}}\;,
	\end{align*}
	where the term $\mathsf{error}(v,k)$ represents a $\mathcal{F}_{\tau_{k-1}}$-measurable  random variable bounded by $e^{-k^\delta}, \Pd_{T_0,x;\mathcal{L}}$-almost surely. 
\end{lemma}}
Again, we will defer the proof of the above lemma to the end of this section. Now we will show how Theorem \ref{thm:powerlaw} follows from the aforementioned lemmas.
\begin{proof} [Proof of Theorem \ref{thm:powerlaw}] We begin by noticing that, if $N_k(d)$ denotes the number of vertices of degree $d$ in $\widetilde{T}_k$ (ignoring the colors), then  for all~$d\in \mathbb{N}\setminus \{0\}$ \com{we need not define $N_k(d)$!},
% \begin{equation}\label{eq:boundNd}
% \frac{\sum_{v\in \widetilde{\vertexset{}}_k} \mathbb{1}\{b_k(v)=d, v\text{ is blue}\}}{k} \le \frac{N_k(d)}{k} %\le \frac{B_k(d)}{k} + \frac{R_k}{k}\;,
% \end{equation}
%\comj{In the first numerator we have the number of vertices which have $d$ blue and zero red half-edges. This is bounded by $B_k(d)$ itself, no? So inside the absolute value below the quantity is non-positive. So I would rather say simply this: 
\begin{align}\label{first.easy}
    0\le B_k(d)-\sum_{v\in \widetilde{\vertexset{}}_k} \mathbb{1}\{b_k(v)=d, v\text{ is blue}\} \le R_k\;.
\end{align}
 
% and thus
% $$\left | \frac{\sum_{v\in \widetilde{\vertexset{}}_k} \mathbb{1}\{b_k(v)=d, v\text{ is blue}\} - B_k(d)}{k} \right| \le \frac{R_k}{k}\;.
% $$ 

Note also that 
\begin{align}\label{second.easy}
    0\le \sum_{v\in \widetilde{\vertexset{}}_k}\mathbb{1}\{\degree{\widetilde{T}_k}{v} = d\}-\sum_{v\in \widetilde{\vertexset{}}_k} \mathbb{1}\{b_k(v)=d, v\text{ is blue}\}\le R_k\;.
\end{align}
By virtue of Lemma~\ref{lemma:Rk}, $\lim_k R_k/k=0,\ \Pd_{T_0,x;\mathcal{L}}$-a.s. Putting this together with \eqref{first.easy} and \eqref{second.easy}, we see that in order to prove  Theorem~\ref{thm:powerlaw}, it is enough to show the following claim.

\medskip 
%
\begin{claim}[Limit distribution for blue degrees]\label{Bk} For any  $d \in \mathbb{N}\setminus \{0\}$,
	\begin{equation*}
	\lim_{k \rightarrow \infty} \frac{B_k(d)}{k} = \frac{4}{d(d+1)(d+2)}\;, \quad  \Pd_{T_0,x; \mathcal{L}}\text{-a.s.}
	\end{equation*}
\end{claim}

%The proof of the above claim relies on  stochastic approximation technique \cite{} \com{we should cite something} to deal with the error arising from the fact that 
%the blue degree of a vertex does not evolve according to a ``pure'' linear preferential attachment scheme, i.e., the probability of a vertex increasing its blue degree by one  is not simply proportional to its blue degree, but there is an error which must be bounded. 
%
%To keep the paper self-contained, we state below the result we shall use, which is taken ``ad litteram'' from \cite{dereich2014robust}. 

%\begin{lemma}[Lemma~3.1 in  \cite{dereich2014robust}]\label{lem:approximation}
%	Let $\{Q_n\}_{n\geq 0}$ be a non-negative stochastic process satisfying the following recursion:
%	\[
%	Q_{n} - Q_{n-1} = \frac{1}{n} \left( \Psi_{n-1} -Q_{n-1} \Phi_{n-1} \right) +  M_{n}- M_{n-1}\;,
%	\]
%	where, $\{\Psi_{n}\}_{n\geq 0}, \{\Phi_{n}\}_{n\geq 0}$ are almost-surely convergent processes with deterministic limits $\psi>0$ and $\phi>0$, respectively, and $\{M_{n}\}_{n\geq 0}$ is an almost-surely convergent process. Then, $\lim_{n \to \infty}Q_n= \psi/\phi$, almost surely.
%\end{lemma}

\begin{claimproof} 
We want to show that the evolution of the blue degrees behaves much like a preferential attachment scheme. This is not a-priori clear because mixing on a long ``good'' time interval only yields\footnote{Since the stationary distribution on a fixed graph is proportional with the degrees.} that the full degrees (including the red degrees) of the vertices behave like that scheme. However, we are going  to show that the value of
\begin{equation*}
	\Pd_{T_0,x;\mathcal{L}}\left( \Delta b_k(v) = 1 \mid\Delta \tau_k \text{ is good}, \widetilde{\mathcal{F}}_{k-1}\right) \;,
	\end{equation*}
	is ``close'' to 
$\frac{b_{k-1}(v)}{2(k-1)}$, where here and in the sequel, $v\in \widetilde{\mathcal{V}}_{k-1}$. This means that $v$ receives the new blue half edge (if there is one) with a probability that is roughly proportional to its existing blue degree.

In order to achieve this, by Lemma \ref{lemma:xtaucond} and recalling that $\Delta \tau_k$ is good if $\Delta \tau_k \ge k^{2+\delta}+1$ \com{if $\Delta \tau_k \ge k^{1+\delta/2}\cdot {\rm diam}(\widetilde{T}_{k-1})+1$}, we have that
	\begin{align}\label{eq:xvdeg}
	\Pd_{T_0,x;\mathcal{L}}\left( X_{\tau_{k} - 1}  = v  \mid \Delta \tau_k \text{ is good}, \mathcal{F}_{\tau_{k-1}}\right) =\frac{\degree{\tau_{k-1}}{v}}{2(k-1)} + \mathsf{error}(v,k)\;, \; \Pd_{T_0,x;\mathcal{L}}\text{-a.s.} 
	\end{align}
	Where $\mathsf{error}(v,k)$ represents a $\mathcal{F}_{\tau_{k-1}}$-measurable random variable bounded by \com{$e^{-k^{\delta/2}}$} $e^{-k^\delta}, \Pd_{T_0,x;\mathcal{L}}$-almost surely. %
	From the definition of the color-assignment process, we have that 
	$$
	\Pd_{T_0,x;\mathcal{L}}\left( \Delta b_k(v) = 1 \mid  X_{\tau_{k} - 1}  = v,\Delta \tau_k \text{ is good}, \widetilde{\mathcal{F}}_{k-1}\right) = \frac{B_{k-1}}{2(k-1)}\;,$$ 
	which, combined with  \eqref{eq:xvdeg}, and using that  $\degree{\tau_{k-1}}{v}=b_{k-1}(v) + r_{k-1}(v)$  and $B_k +R_k = 2k$, leads to
	%
	\begin{equation}\label{eq:prob_increments}
	\begin{split}
	&\Pd_{T_0,x;\mathcal{L}}\left( \Delta b_k(v) = 1 \mid \Delta \tau_k \text{ is good}, \mathcal{F}_{\tau_{k-1}}\right)=
	\\
	&\qquad \frac{b_{k-1}(v)}{2(k-1)} + \underbrace{ \frac{B_{k-1}r_{k-1}(v) - b_{k-1}(v)R_{k-1}}{(2(k-1))^2} \pm \frac{B_{k-1}}{2(k-1)}\mathsf{error}(v,k)}_{:=F_{k-1}(v)}\;,
	\end{split}
	\end{equation}
% 	\begin{equation}\label{eq:prob_increments}
% 	\begin{split}
% 	\Pd_{T_0,x;\mathcal{L}}\left( \Delta b_k(v) = 1 \mid\Delta \tau_k \text{ is good}, \widetilde{\mathcal{F}}_{k-1}\right) & = \frac{b_{k-1}(v)}{2(k-1)} + F_{k-1}(v)\;,
% 	\end{split}
% 	\end{equation}
	where $F_{k-1}(v)$ is a $\widetilde{\mathcal{F}}_{k-1}$-measurable random variable satisfying that
	\begin{equation}\label{eq:Forder}
	F_{k-1}(v) = \mathcal{O}\left( \frac{B_{k-1}r_{k-1}(v)-b_{k-1}(v)R_{k-1}}{(k-1)^2}\right)\;.
	\end{equation}
	Here $\mathcal{O}$ refers to a limit as $k\to\infty$. Note that although the collection of $v$'s to which this applies, keeps changing, the term $\mathsf{error}(v,k)$  is uniformly bounded in $v$.
	Denote by $\mathcal{B}_k(d)$ the subset 
	of vertices in $\widetilde{\vertexset{}}_k$ whose blue degree is exactly $d$;
   note that  $|\mathcal{B}_k(d)|={B}_k(d)$. Clearly,
   
	\begin{align*}
	% \Delta B_k(1)&=
	%  1 - \sum_{v \in \widetilde{\vertexset{}}_{k-1}} \mathbb{1}\left\{ \Delta b_{k}(v)=1\right \}\mathbb{1}\left\{  b_{k-1}(v)=1\right \}   
	% \\
	\Delta B_k(d)=\begin{cases}
	\mathbb{1}\{\Delta \tau_{k} \text{ is good} \} + {\!\!\displaystyle\sum_{v \in \mathcal{B}_{k-1}(0)} \!\!\mathbb{1}\left\{ \Delta b_{k}(v)=1\right \}} - \!\!\displaystyle\sum_{v \in \mathcal{B}_{k-1}(1)} \!\!\mathbb{1}\left\{ \Delta b_{k}(v)=1\right \}  \;, & d=1\;,
	\\[7pt]
	% = \sum_{v \in \widetilde{\vertexset{}}_{k-1}} \mathbb{1}\left\{ b_{k}(v)=d\right \} - \mathbb{1}\left\{ b_{k-1}(v)=d\right \}
	% \\
	% &
	\!\displaystyle\sum_{v \in \mathcal{B}_{k-1}(d-1)} \!\!\mathbb{1}\left\{ \Delta b_{k}(v)=1\right \}-\sum_{v \in \mathcal{B}_{k-1}(d)} \!\!\mathbb{1}\left\{ \Delta b_{k}(v)=1\right \}\;, & d>1\;.
	% - \sum_{v \in \widetilde{\vertexset{}}_{k-1}} \mathbb{1}\left\{ \Delta b_{k}(v)=1\right \}\mathbb{1}\left\{  b_{k-1}(v)=d\right \}
	\end{cases}
	\end{align*}
     To avoid clutter, henceforth we set  
	$$
	W_{k-1}:= \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}\mid  \mathcal{F}_{\tau_{k-1}}\right).
	$$ 
	Notice that for $v \in \mathcal{B}_{k-1}(0)$ Equation \eqref{eq:prob_increments} gives us that 
	$$
	    \Pd_{T_0,x;\mathcal{L}}\left( \Delta b_k(v) = 1 \mid \Delta \tau_k \text{ is good}, \mathcal{F}_{\tau_{k-1}}\right) = F_{k-1}(v)\;,
	$$
	which together with the fact vertices can increase their blue degree only at good times, $B_k \le 2k$ and  \eqref{eq:Forder} implies that 
	\begin{equation*}\label{eq:Fbk0}
	\Ed_{T_0,x;\mathcal{L}}\left[\sum_{v \in \mathcal{B}_{k-1}(0)} \mathbb{1}\left\{ \Delta b_{k}(v)=1\right \} \middle | \widetilde{\mathcal{F}}_{k-1}\right] = W_{k-1}\sum_{v \in \mathcal{B}_{k-1}(0)}F_{k-1}(v)  =  W_{k-1}\mathcal{O}\left(\frac{R_{k-1}}{k-1}\right).
	\end{equation*}
	Then,  using the above identity and \eqref{eq:prob_increments} we obtain 
	\begin{equation}\label{eq:average_increments}
	\begin{split}
	% \Ed_{T_0,x; \mathcal{L}}\left(\Delta B_k(1) \mid  \mathcal{F}_{\tau_{k-1}}\right)&=
	% W_{k-1} \left( 1 -  \frac{B_{k-1}(1)}{2(k-1)} - Y_{k-1}(1)\right)
	% % \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)
	% \;,
	% \\
	\Ed_{T_0,x;\mathcal{L}}\left[\Delta B_k(d) \mid \widetilde{\mathcal{F}}_{k-1}\right] &=
	W_{k-1}\, \frac{(d-1)B_{k-1}(d-1)- d\, B_{k-1}(d)}{2(k-1)}\\
	& \quad + W_{k-1}\left(Y_{k-1}(d-1) 
	- Y_{k-1}(d) \right)\;,
	%  \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)
	%  \\
	% & \qquad - \left( d\,\frac{B_{k-1}(d)}{2(k-1)} \pm Y_{k-1}(d)\right) \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)\;, 
	\end{split}
	\end{equation}
	where, $Y_{k-1}(0)\equiv1$ and  for every $d\geq 1$,
	\begin{align}\label{eq:Yd}
	Y_{k-1}(d):=\begin{cases}
	\sum_{v \in \mathcal{B}_{k-1}(d)} F_{k-1}(v) - \sum_{v \in \mathcal{B}_{k-1}(0)} F_{k-1}(v)\;, & d =1\;, \\
	    \sum_{v \in \mathcal{B}_{k-1}(d)} F_{k-1}(v)\;, & d>1\;.
	    \end{cases}
	% \begin{cases}
	% \frac{B_{k-1}}{2(k-1)}\displaystyle\sum_{v \in \widetilde{\vertexset{}}_{k-1}} \mathbb{1}\left\{  b_{k-1}(v)=1\right \}\left( \frac{r_{k-1}(v)}{2(k-1)} \pm \mathrm{error}(v,k) \right) - \frac{B_{k-1}(1)R_{k-1}}{(2(k-1))^2} \;, & d=1\;,
	% \\
	% % \sum_{v \in \widetilde{\vertexset{}}_{k-1}}\mathbb{1}\left\{  b_{k-1}(v)=d-1\right \}\left(\frac{B_{k-1}r_{k-1}(v) - b_{k-1}(v)R_{k-1}}{(2(k-1))^2} \pm \frac{B_{k-1}}{2(k-1)}\mathrm{error}(v,k)\right)
	% % \\
	% % &
	% % =
	% \frac{B_{k-1}}{2(k-1)}\displaystyle\sum_{v \in \widetilde{\vertexset{}}_{k-1}} \mathbb{1}\left\{  b_{k-1}(v)=d\right \} \left( \frac{r_{k-1}(v)}{2(k-1)} \pm \mathrm{error}(v,k) \right) - d\frac{B_{k-1}(d)}{(2(k-1))^2}\;, & d>1\;.
	% \end{cases}
	\end{align}
	Notice that for all $d\ge 1$, by \eqref{eq:Forder} we have that 
	$$
	    Y_{k-1}(d) = \mathcal{O}\left( \frac{R_{k-1}}{k-1}\right).
	$$
	
	Now, in order to simplify our notation, set $Q_{k}(d):= B_k(d)/k$. Then, writing 
	$$
	Q_k(d) - Q_{k-1}(d) = Q_k(d) - \Ed_{T_0,x; \mathcal{L}}\left[Q_k(d) \mid \widetilde{\mathcal{F}}_{k-1}\right] + \Ed_{T_0,x; \mathcal{L}}\left[Q_k(d) \mid  \widetilde{\mathcal{F}}_{k-1}\right] - Q_{k-1}(d)\;,
	$$
	and applying  \eqref{eq:average_increments}, we obtain the following recursion for~$Q_k(d)$:
	% \begin{align*}
	% Q_{k}(d) - Q_{k-1}(d)= M_k(d)  +   \Ed_{T_0,x; \mathcal{L}}\left( Q_{k}(d) \mid  \mathcal{F}_{\tau_{k-1}}\right) - Q_{k-1}(d)\;,
	% \end{align*}
	% where $M_k(d):= Q_{k}(d) -  \Ed_{T_0,x; \mathcal{L}}\left( Q_{k}(d) \mid  \mathcal{F}_{\tau_{k-1}}\right) $ is a martingale and for $d=1$ we have  
	% \begin{align*}
	% &\Ed_{T_0,x; \mathcal{L}}\left( Q_{k}(1) \mid  \mathcal{F}_{\tau_{k-1}}\right) - Q_{k-1}(1) =  - \frac{B_{k-1}(1)}{(k-1)}\frac{\Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)}{2(k-1)} 
	% \\&-\left(1 - \frac{\Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)}{2(k-1)}\right) \frac{B_{k-1}(1)}{(k-1)k} 
	%  + (1\pm Y_{k-1}) \frac{\Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)}{k}
	% \\
	% &= \frac{1}{k} \left( (1\pm Y_{k-1}) \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right) - Q_{k-1}(1) \left( 1 + \frac{\Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)}{2}
	% % + \frac{\com{k}\Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)}{2(k-1)} 
	% \right)\right) 
	% \end{align*}
	% whereas for $d>1$ we have  \com{check}
	% \begin{align*}
	% &\Ed_{T_0,x; \mathcal{L}}\left( Q_{k}(d) \mid  \mathcal{F}_{\tau_{k-1}}\right) - Q_{k-1}(d) = 
	% % - \frac{B_{k-1}(1)}{2(k-1)k} - \frac{\Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)}{2k} \frac{B_{k-1}(1)}{2(k-1)k} 
	% % \\
	% % &\qquad \qquad + (1\pm Y_{k-1}) \frac{\Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)}{2k}
	% \\
	% & \frac{1}{k} \Bigg( \left( \frac{d-1}{2}\, Q_{k-1}(d-1) \pm Y'_{k-1} \pm Y_{k-1}\right) \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)
	% \\
	% &- Q_{k-1}(d) \left( 1 + d\,\frac{\Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)}{2}\right)\Bigg) 
	% \end{align*}
	% For every $d\in \mathbb{N}\setminus \{0\}$, and for every $k$, $Q_k(d)$ satisfies 
	\begin{align}\label{eq:decomposition_lemma}
	Q_{k}(d) - Q_{k-1}(d) = \frac{1}{k} \left( \Psi_{k-1}(d-1) -Q_{k-1}(d) \Phi_{k-1}(d) \right) + \Delta M_{k-1}(d)\;,
	\end{align}
	where, for every $d\geq 1$, we have that 
	\begin{itemize}
		\item $\Psi_{k-1}(d-1)=\Big(\frac{d-1}{2}Q_{k-1}(d-1) + Y_{k-1}(d-1) - Y_{k-1}(d)\Big)
		W_{k-1}$;
		\item $\Phi_{k-1}(d)= 1 + \frac{d}{2}W_{k-1} = 1 + \frac{d}{2}\Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}\mid  \widetilde{\mathcal{F}}_{k-1}\right)$;
		\item $\Delta M_{k-1}(d) = Q_{k}(d) -  \Ed_{T_0,x; \mathcal{L}}\left[ Q_{k}(d) \mid  \widetilde{\mathcal{F}}_{k-1}\right]$.
	\end{itemize}
	In light of Lemma \ref{lem:approximation}, our goal is to guarantee that both of the processes~$\{\Psi_{n}(d-1)\}_{n\ge 0}$ and $\{\Phi_{n}(d)\}_{n\ge 0}$ have positive and deterministic limits and $\{M_n(d)\}_{n\geq 0}$ is convergent, for all fixed $d$.
	 
	The convergence of $\{\Phi_{n}(d)\}_{n\ge0}$ to $1+d/2$ (i.e. that $W_{k-1} \to 1$) comes as a consequence of Lemma~\ref{lemma:limtauk}. Indeed, observe that
	$$
	W_{k-1} = \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \ge k^{2+\delta}+1\mid  \mathcal{F}_{\tau_{k-1}}\right) = \prod_{s=\tau_{k-1}+1}^{\tau_{k-1}+k^{2+\delta}+2}(1-p_s) \to 1\;,
	$$
	$\Pd_{T_0,x;\mathcal{L}}$-a.s. as $k$ goes to infinity, since $p_s = \Theta(s^{-\gamma})$ and by Lemma~\ref{lemma:limtauk}, $k^{2+\delta}/\tau_k^{\gamma}$ goes to zero almost surely.
	
	\com{
		The convergence of $\{\Phi_{n}(d)\}_{n\ge0}$ to $1+d/2$ (i.e. that $W_{k-1} \to 1$ a.s.) follows from observing that 
	$$
	W_{k-1} = 1 -  \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is bad}\mid  \mathcal{F}_{\tau_{k-1}}\right) \;,
	$$
	and as shown in~\eqref{eq:badtau}, by Theorem~\ref{thm:diam} and Lemma~\ref{lemma:limtauk}, $\Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is bad}\mid  \mathcal{F}_{\tau_{k-1}}\right)$ goes to zero, 
	$\Pd_{T_0,x;\mathcal{L}}$-a.s., as $k$ goes to infinity.
	}
% 	Next we will deal with the process $\{M_n(d)\}_{n\geq 0}$.\\
	
	\medskip 
	
	\noindent \underline{Convergence of $\{M_n(d)\}_{n\geq 0}$:} For a fixed $d$, the terms $\Delta M_{k}(d)$ define a martingale difference sequence. Setting~$M_0(d)= 0$, let the process $\{M_n(d)\}_{n\geq 0}$ be the corresponding martingale. Diving both sides of  \eqref{eq:average_increments} yields to
	$$
	    \Ed_{T_0,x; \mathcal{L}}\left[ Q_{k}(d) \mid  \widetilde{\mathcal{F}}_{k-1}\right] = \frac{B_{k-1}(d)}{k} + \mathcal{O}\left(\frac{B_{k-1}(d) + B_{k-1}(d-1)+ R_{k-1}}{k^2 }\right),
	$$
	which implies that
	\begin{equation*}
	\begin{split}
	|\Delta M_{k-1}(d) | = \frac{\Delta B_k(d)}{k}+\mathcal{O}\left(\frac{B_{k-1}(d) + B_{k-1}(d-1)+ R_{k-1}}{k^2 }\right)\;.
	\end{split}
	\end{equation*}
	On the other hand, since $\Delta B_k(d) \le 2$ and $B_k(d)$ and $R_k$ are less than~$2k$ for all $d$, it follows that
	\begin{align*}
    (\Delta M_k(d))^2 = 
	\mathcal{O}\left(\frac{1}{k^2}\right),
	\end{align*}
	which is sufficient to guarantee that $\{M_n(d)\}_{n\geq 0}$ is bounded in $L^2$ and thus converges $\Pd_{T_0,x;\mathcal{L}}$-almost surely. \\
	%
	% \begin{align*}
	% & \Psi_{k-1}(d-1)=\Big(\frac{d-1}{2}Q_{k-1}(d-1) + Y_{k-1}(d-1) - Y_{k-1}(d)\Big)
	% W_{k-1}
	% = \begin{cases} \Big(\frac{d-1}{2}Q_{k-1}(d-1) + Y_{k-1}(d-1) - Y_{k-1}(d)\Big)
	% W_{k-1}\;,
	% % \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)
	% & d>1\;,
	% \\[8pt]
	% \left(1\pm Y_{k-1}(1)\right)W_{k-1}\;,
	% % \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)
	% & d=1\;,
	%     \end{cases}
	%     \\
	% &\Xi_{k-1}(d)= 1 + \frac{d}{2}W_{k-1}\;,
	% % \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}|  \mathcal{F}_{\tau_{k-1}}\right)
	% \\
	% & \Delta M_{k-1}(d) = M_k(d)-M_{k-1}(d):= Q_{k}(d) -  \Ed_{T_0,x; \mathcal{L}}\left( Q_{k}(d) \mid  \mathcal{F}_{\tau_{k-1}}\right)\;,
	% \end{align*}

	\noindent \underline{Convergence of $\{\Psi_{k}(d-1)\}_{k\ge 0}$:} This part requires induction on $d$, since $\Psi_{k}(d-1)$ is defined via $Q_{k}(d-1)$. Thus, our first step is to prove it for $d=1$.
	
	Observe that as a consequence of Lemma~\ref{lemma:Rk} and  \eqref{eq:Yd}, we have that $\{Y_n(d)\}_n$ converges to zero for $d\ge 1$. Moreover, when $d=1$, Lemma~\ref{lemma:limtauk} implies that 
%	To show  that, for all $d \in \mathbb{N}\setminus \{0\}$, $\lim_{k \to \infty} Q_k(d)= \frac{4}{d(d+1)(d+2)}$ almost surely,  we recursively apply Lemma~\ref{lem:approximation} to Equation~\eqref{eq:decomposition_lemma}. Specifically,  for $d=1$, using that 
	\begin{align*}
	\lim_{k \rightarrow \infty}\Psi_{k-1}(0)&=    \lim_{k \rightarrow \infty}(1 -Y_{k-1}(1)) \Pd_{T_0,x;\mathcal{L}}\left(\Delta \tau_k \text{ is good}\mid   \widetilde{\mathcal{F}}_{k-1}\right) = 1\;.
	\end{align*}
	Combining the above with our previous results and Lemma~\ref{lem:approximation} gives us that $\{Q_n(1)\}_{n\ge 0}$ converges to $\frac{1}{1+1/2}=2/3$.
	%
	Now let $d\ge 2$. Using induction we show that $\lim_{k\to \infty}Q_{k}(d)$ exists a.s., and calculate the limit recursively. So let us assume  that $\lim_{k\to \infty}Q_k(d-1)=:Q(d-1)$ exists almost surely.  It follows that $$\lim_{k\to \infty}\Psi_k(d-1)=(d-1)Q(d-1)/2,\ \text{a.s.}$$  Using  Lemma~\ref{lem:approximation} again,  we conclude  that 
	\[
	Q(d):=\lim_{k\to \infty}Q_{k}(d) = \frac{\frac{d-1}{2}\cdot Q(d-1)}{(1+ d/2)} =\frac{d-1}{d+2}\cdot Q(d-1) \;, \quad \text{ $\Pd_{T_0,x;\mathcal{L}}$-a.s.}
	\]
	which implies that for $d\geq 1$,  $$\lim_{k\to \infty}Q_{k}(d)=\frac{4}{d(d+1)(d+2)},\quad\mathbb{P}_{T_0,x; \mathcal{L}}\text{-a.s.}$$ and proves Claim \ref{Bk}.
\end{claimproof}

\medskip
Returning now to the proof of Theorem~\ref{thm:powerlaw}, recall that, as observed at the beginning of our argument, the statement follows from  Claim \ref{Bk}, and we are done.
\end{proof}

\medskip 
Finally, having shown how Theorem \ref{thm:powerlaw} follows from our lemmas, we still owe the proofs of Lemmas \ref{lemma:limtauk}, \ref{lemma:Rk} and \ref{lemma:xtaucond}, and this is what we are going to do below.
\begin{proof}[Proof of Lemma~\ref{lemma:limtauk}]
% Let us begin by noticing that the claim is true for $\gamma>1$, since in this regime one has $\tau_k=+\infty$, for all sufficiently large $k$, $\Pd_{T_0,x;\mathcal{L}}$-a.s. In the sequel, we therefore address the case $\gamma \in (2/3,1]$ \com{$\gamma \in (1/2,1]$}.
Let $V_m=|\vertexset{m}|$ and note that  $V_m := Z_1 +\dots +Z_m$, which implies that, as $m\to\infty$, \[
\Ed_{T_0, o;\mathcal{L}}(V_m) = \Theta (m^{1-\gamma})\;.
\]
Since $\tau_{k}$ is the first time of having $k+1$ vertices, if $T_0=\{o\}$, one has the identity
\begin{equation*}
\Lbrace \tau_{k} \le k^{1 /(1-\gamma) 
-\varepsilon
} \Rbrace = \Lbrace V_{k^{1 /(1-\gamma) 
-\varepsilon
}} \ge k\Rbrace\;,
\end{equation*}
 for any $\varepsilon < 1/(1-\gamma)$.
Recalling  the independence of the $Z_n$'s, using that $\log(1+x)<x,\ x>0$,  and bounding the sum by an integral, it follows that for every $\lambda>0$,
\begin{equation*}
\log\Ed_{T_0,x;\mathcal{L}} \left( e^{\lambda V_m}\right) \le \begin{cases}
 (e^{\lambda}-1)m^{1-\gamma}/(1-\gamma)\;, & \gamma <1\;,
\\
(e^{\lambda}-1)(\log m + 1) \;, & \gamma =1\;. 
\end{cases}
\end{equation*}
Thus, by the exponential Markov inequality  there is a positive constant $C$ depending on~$\gamma$ only, such that
\begin{equation}\label{two.exp}
\begin{split}
\Pd_{T_0,x;\mathcal{L}} \left( V_{k^{ 1/(1-\gamma) -\varepsilon}} \ge k \right)\le e^{-k}e^{Ck^{1-(1-\gamma)\varepsilon}}.
\end{split}
\end{equation}
%
This and the Borel-Cantelli lemma yields that $\tau_{k}<k^{1 /(1-\gamma) -\varepsilon}$ occurs only finitely many times, almost surely, \com{thus the same occurs for $\tau_{k}^{\gamma}<k^{\gamma /(1-\gamma) -\gamma\varepsilon}$}. 
% We conclude the proof by choosing a small enough  $\varepsilon>0$ and noting that $\gamma > 2/3$ if and only if $\gamma/(1-\gamma) > 2$ \com{$\gamma > 1/2$ if and only if $\gamma/(1-\gamma) > 1$}. 
\end{proof}
Now we prove Lemma \ref{lemma:xtaucond} first and prove Lemma \ref{lemma:Rk} at the end of this section.
%%% LEMMA:XTAUCOND


\begin{proof}[Proof of Lemma \ref{lemma:xtaucond}]  
	% As a shorthand, let us say $\Delta \tau_k := \tau_k - \tau_{k-1}$ is \textit{good} if it satisfies
	% \begin{equation}\label{def:goodtau}
	% \Delta \tau_k > k^{2+\delta} +1
	% \end{equation}
	% for a fixed $\delta$ that will be chosen properly later. We say $\Delta \tau_k$ is \textit{bad} otherwise.
	%
	%
	%
	%Notice that by the definition of $\tau_k$,  the amount $k$ is exactly the total number of vertices of $T_{\tau_{k-1}}$.
	%
	Recall that $\{\mathcal{G}_n\}_{n\geq 1}$ denotes the natural filtration induced by the variables $\{Z_n\}_{n\geq 1}$. Observe that conditioned on $\mathcal{G}_{k-1}$, $\Delta \tau_k$ dominates a random variable $Y_k$ following geometric distribution of parameter ~$c/\tau_{k-1}^{\gamma}$, where $c$ is a positive constant depending on $(p_n)_n$ only.  Thus,  for $k$ sufficiently large, there exists a positive constant~$C$ such that, almost surely,
	\begin{equation}\label{eq:badtau}
	\begin{split}
	\Pd_{T_0,x;\mathcal{L}}\left( \Delta \tau_k \text{ is bad} \mid  \widetilde{\mathcal{F}}_{k-1} \right) & \le  \Pd_{T_0,x;\mathcal{L}}\left( Y_k < k^{2+\delta} +1 \mid  \widetilde{\mathcal{F}}_{k-1} \right)\le C\frac{k^{2+\delta}}{\tau_{k-1}^{\gamma}}\;.
	\end{split}
	\end{equation}

	\com{
	\begin{equation}\label{eq:badtau}
	\begin{split}
	&\Pd_{T_0,x;\mathcal{L}}\left( \Delta \tau_k \text{ is bad} \mid  \widetilde{\mathcal{F}}_{k-1} \right)  \le  \Pd_{T_0,x;\mathcal{L}}\left( Y_k < k^{1+\delta/2} \cdot {\rm diam}(T_{\tau_{k-1}})+1 \mid  \widetilde{\mathcal{F}}_{k-1} \right)
	\\
	&\leq \Pd_{T_0,x;\mathcal{L}}\left( Y_k < k^{1+\delta/2} \cdot {\rm diam}(T_{\tau_{k-1}})+1, {\rm diam}(T_{\tau_{k-1}})\leq C k^\varepsilon \mid  \widetilde{\mathcal{F}}_{k-1} \right) 
	\\
	& \qquad + \Pd_{T_0,x;\mathcal{L}}\left( {\rm diam}(T_{\tau_{k-1}})> C k ^\varepsilon \mid  \widetilde{\mathcal{F}}_{k-1} \right)
	\\
	&
	\leq \Pd_{T_0,x;\mathcal{L}}\left( Y_k < Ck^{1+\delta/2 + \varepsilon}   +1 \mid  \widetilde{\mathcal{F}}_{k-1} \right) 
	 + \Pd_{T_0,x;\mathcal{L}}\left( {\rm diam}(T_{\tau_{k-1}})> Ck^\varepsilon \mid  \widetilde{\mathcal{F}}_{k-1} \right)
	\\
	&\le C'\frac{k^{1+\delta/2+\varepsilon}}{\tau_{k-1}^{\gamma}}+ \frac{1}{\tau_{k-1}^{M}}\;,
	\end{split}
	\end{equation}
	}
% 	\com{\begin{equation}\label{eq:badtau}
% 	\begin{split}
% 	P\left( \Delta \tau_k \text{ is bad} \mid  \mathcal{G}_{k-1} \right) & \le  \Pd\left( Y_k < k^{2+\delta} +1  \right) \le C\frac{k^{2+\delta}}{\tau_{k-1}^{\gamma}}\;.
% 	\end{split}
% 	\end{equation}}
% 	\comr{It should be $\widetilde{\mathcal{G}}_k$. I put some thought on this notation thing and I don't see why we need to introduce another notation and another filtration. Everything holds true with the stopped natural filtration $\widetilde{\mathcal{F}}_n$ and the larger probability measure $\mathbb{P}$, why should we introduce new stuff to make so simple statement as the one in (3.15)?}
	\com{where in the last inequality (for the second term) we are using Theorem~\ref{thm:diam}.  Chosing $\varepsilon$ sufficently small (smaller than $\delta/2$) and $M\geq\gamma$,  Lemma~\ref{lemma:limtauk} gives us that \st{allows us to choose $\delta$ small enough so} the RHS of the above inequality goes to zero almost surely when $k$ goes to infinity.}
	
	Now, let $\Pi_k$ be the (random) stationary distribution of a simple random walk on the rooted tree $T_{\tau_k}$  with a self-loop attached to the root $o$ (we introduce a self-loop at the root just to avoid periodicity). More specifically, $\Pi_k$ is the random distribution over $\vertexset{\tau_k}$ which assigns to each $v\in \vertexset{\tau_k}$ the weight
	\begin{equation*}
	\Pi_k(v) := \frac{\degree{\tau_{k}}{v}}{2k}\;.
	\end{equation*}
	Let $P_{x, T}^t$ denote the distribution of a random walk over $T$ started at $x$ after $t$ steps. It is known (see \cite{brightwellwinkler1990} \com{to be updated}) that the mixing time of a random walk on a tree $T$ with $k$ vertices satisfies the  upper bound
	\begin{equation}\label{eq:boundtmix}
	\tmix \le  2k^2\;, \com{ \tmix \le  k \cdot{\rm diam}(T)}
	\end{equation}
	uniformly in the initial state $x\in T$. Recall that $\rm d_{\rm TV}$  denotes the total variation distance. It is well known that for any $\varepsilon>0$ the  upper bound  
	\begin{equation*}%\label{eq:tmixeps}
	\tmix(\varepsilon) \le \log\left(\frac{1}{\varepsilon}\right)\tmix \;,
	\end{equation*}
	holds, and
	in particular, for $\varepsilon := \exp\{-k^\delta\}$  by \eqref{eq:boundtmix}, we obtain  that  
	\begin{equation}\label{eq:dtvpt}
	\begin{split}
	\dtv{\Pi_{k-1}}{P^{t}_{X_{\tau_{k-1}}, T_{\tau_{k-1}}}} \le  e^{-k^\delta},\qquad \Pd_{T_0,x;\mathcal{L}}\text{-a.s.}
	\end{split}
	\end{equation}
	for all $t > k^{2+\delta}$ \com{$t > k^{1+\delta}\cdot{\rm diam}(T_{\tau_{k-1}})$}. 
	%
	Next, the Strong Markov property applied to $\mathcal{L}$-\name at time $\tau_{k-1}$ yields
	\begin{equation}\label{eq:markov}
	\Pd_{T_0,x;\mathcal{L}}\left( X_{\tau_{k} - 1} = v \mid \mathcal{F}_{\tau_{k-1}}\right) = \Pd_{X_{\tau_{k-1}}, T_{\tau_{k-1}}; \mathcal{L}^{(\tau_{k-1})}} \left( X_{\tau_1 -1} = v\right)\;.
	\end{equation} 
	% To simplify the notation let $\bar{\Pd}$ be a shorthand to the random distribution $\Pd_{X_{\tau_{k-1}}, T_{\tau_{k-1}}, Z\circ \widetilde{\theta}_{k-1}}$. 

	Observe that under $\Pd_{X_{\tau_{k-1}}, T_{\tau_{k-1}}; \mathcal{L}^{(\tau_{k-1})}}$ conditioned on  $\tau_1 = t$, $X_{\tau_1 -1}$ has distribution $P^{t}_{X_{\tau_{k-1}}, T_{\tau_{k-1}}}$. The reader may check this fact recalling that the event $\tau_1 = t$ depends only on the random variables $\{Z_n\}_{n\geq 1}$ together with  the independence of $Z_n$ from $\mathcal{F}_{n-1}$, for all $n$. 
	
	Using  \eqref{eq:markov} and \eqref{eq:dtvpt} for $t>k^{2+\delta}$ \com{$t > k^{1+\delta}\cdot {\rm diam}(T_{\tau_{k-1}})$}, we have that
	\begin{equation*}
	\Pd_{X_{\tau_{k-1}}, T_{\tau_{k-1}}; \mathcal{L}^{(\tau_{k-1})}}\left( X_{\tau_1 -1 } = v\mid \tau_1 = t\right) = \frac{\degree{\tau_{k-1}}{v}}{2(k-1)} \pm \mathsf{error}(v,k)\;,
	\end{equation*}
	where $\mathsf{error}(v,k)$ represents an $\mathcal{F}_{\tau_{k-1}}$-measurable  random variable for which 
	\[
	\Pd_{T_0,x;\mathcal{L}}\left(\mathsf{error}(v,k)\le e^{-k^\delta}\right)=1\;.
	\]
This concludes the proof.
	\end{proof}


%%%%%%%% LEMMA:Rk %%%%%%%%%%%%%%%%
\begin{proof}[Proof of Lemma~\ref{lemma:Rk}] We know that  $\Delta R_k=2$  when $\Delta\tau_{k}$ is bad, while it equals $1$ when  $\Delta\tau_{k}$ is good and the half-edge $h_{k,2}$ is colored red. Therefore, 
	\begin{equation}\label{eq:expecdeltar}
	\begin{split}
	&\Ed_{T_0,x;\mathcal{L}} \left[\Delta R_k \mid
	\mathcal{F}_{\tau_{k-1}}
	%\widetilde{\mathcal{F}}_{k-1} 
	\right]\\
	 &=  2\Pd_{T_0,x;\mathcal{L}} \left( \Delta\tau_{k}\text{ is bad}\mid 
	\mathcal{F}_{\tau_{k-1}}
	%\widetilde{\mathcal{F}}_{k-1}
	\right)+ \frac{R_{k-1}}{2(k-1)}\Pd_{T_0,x;\mathcal{L}} \left( \Delta\tau_{k}\text{ is good}\mid
	\mathcal{F}_{\tau_{k-1}}
	%\widetilde{\mathcal{F}}_{k-1}
	\right) \\
	& = \frac{R_{k-1}}{2(k-1)} + \mathsf{error}(k)\;,
	\end{split}
	\end{equation}
where, $\mathsf{error}(k)$ is an $\mathcal{F}_{\tau_{k-1}}$-measurable variable such that 
\begin{equation}\label{eq:bounderrobad}
 |\mathsf{error}(k)| \le 2\Pd_{T_0,x;\mathcal{L}} \left( \Delta\tau_{k}\text{ is bad}\mid
 \mathcal{F}_{\tau_{k-1}}
% \widetilde{\mathcal{F}}_{k-1}
 \right), \; \Pd_{T_0,x;\mathcal{L}}\text{-a.s.}\;
\end{equation}
Now, define the function $\phi: \{2,3,,...\}\to (1,\infty)$ by 
\begin{equation*}%\label{def:phi}
\phi (k):= \prod_{j=1}^{k-1}\left(1+\frac{1}{2j}\right) =2^{1-k}\frac{(2k-1)!!}{(k-1)!}= \Theta(\sqrt{k})\;,
\end{equation*}
where the last step uses Stirling's formula and that $(2k-1)!!=\frac{(2k)!}{2^{k}k!}$.
In fact, even $\phi (k)/\sqrt{k}\to \text{const}$, which can be computed.
Let 
$R'_k := \frac{R_k}{\phi(k)}$.
%
Using \eqref{eq:expecdeltar}, a simple computation shows that
\begin{equation*}
\Ed_{T_0,x;\mathcal{L}} \left[\Delta R'_k \mid
 \mathcal{F}_{\tau_{k-1}}
% \widetilde{\mathcal{F}}_{k-1} 
\right] = \frac{\mathsf{error}(k)}{\phi(k)}\;.
\end{equation*}
Next, exploiting Doob's decomposition, we may write $R'_k$ as
\begin{equation}\label{Doob.decomp}
R'_k = M_k + \sum_{m=1}^{k} \frac{\mathsf{error}(m)}{\phi(m)}\;,
\end{equation}
where the process $M$ is a mean zero martingale whose increments satisfy that
\begin{equation*}
|M_{j+1} - M_j | = \left | \frac{R_{j+1} -(1+\frac{1}{2j})R_j - \mathsf{error}(j+1)}{\phi(j+1)} \right | \le \frac{5}{\phi(j+1)}\;, \; \Pd_{T_0,x;\mathcal{L}}\text{-a.s.}
\end{equation*}
Thus, there exists a positive constant $C_1$ such that
\begin{equation}\label{the.bound}
\sum_{j=1}^k |M_{j+1} - M_j |^2 \le C_1\log k\;.
\end{equation}
Combining \eqref{the.bound} with the Azuma–Hoeffding inequality \cite{BBD2015Ineq} yields a positive constant $C_2$ depending on $\gamma$ and $C_1$ such that 
\begin{equation*}
\Pd_{T_0,x;\mathcal{L}} \left( M_k > C_2 k^{\delta'/2}\log^{1/2} k \right) \le e^{-k^{\delta'}}\;.
\end{equation*}
To control the predictable term in Doob's decomposition (i.e. the sum in \eqref{Doob.decomp}), we break the sum into two terms as $\sum_{m=1}^{k^{\delta'}}+\sum_{j=k^{\delta'}}^k$, by fixing some $\delta'$ to be chosen later. For the first sum we have the  deterministic bound
\begin{equation*}
\begin{split}
\sum_{m=1}^{k^{\delta'}}\frac{\mathsf{error}(m)}{\phi(m)} \le 2\sum_{m=1}^{k^{\delta'}} \frac{1}{\phi(m)} \le C_3k^{\delta'/2}\;,
\end{split}
\end{equation*}
for some universal constant $C_3$. For the rest of the terms, recall from the proof of Lemma~\ref{lemma:limtauk} (see \eqref{two.exp}) that for any $\varepsilon'<1/(1-\gamma)$ and for large enough $j$,
\begin{equation}\label{eq:boundtj}
\Pd_{T_0,x;\mathcal{L}} \left( \tau_{j} \le j^{1 /(1-\gamma) -\varepsilon'}\right) \le e^{-C_4j}\;.
\end{equation}
Thus, recalling  \eqref{eq:bounderrobad} and \eqref{eq:badtau}, on the event $\bigcap_{j=k^{\delta'}}^k \Lbrace \tau_{j} \ge j^{1 /(1-\gamma) -\varepsilon'} \Rbrace$ we have that
\begin{equation*}
\sum_{j=k^{\delta'}}^k \frac{\mathsf{error}(j)}{\phi(j)} \le \sum_{j=k^{\delta'}}^k C_5 j^{2+\delta - (\gamma/(1-\gamma) -\gamma\varepsilon') -1/2} \le C_6k^{1/2 -\varepsilon}\;,
\end{equation*}
where $\varepsilon>0$  depends on $\gamma$, which is fixed and on $\delta$ and $\varepsilon'$, which can be chosen properly. On the other hand, by the union bound and  \eqref{eq:boundtj} we obtain that 
$$
\Pd_{T_0,x;\mathcal{L}} \left( \bigcup_{j=k^{\delta'}}^k\Lbrace \tau_{j}
\le j^{1 /(1-\gamma) -\varepsilon'} \Rbrace\right) \le \exp\{-C_7k^{\delta'}\}\;.
$$
Since $R_k = R'_k\phi(k)$, it follows that, on the  event  $$\{ M_k \le C_2k^{\delta'/2}\log^{1/2} k\}\,\cap\,\bigcap_{j=k^{\delta'}}^k \Lbrace \tau_{j} \ge j^{1 /(1-\gamma) -\varepsilon'} \Rbrace\;,$$
 the estimate $R_k \le k^{1-\varepsilon}$ holds, which is enough to conclude the proof. 
\end{proof}

\newpage

\textcolor{purple}{\bf TAKEN OUT}\\
Looking at the power of $n$ first, this requires (after some algebra) that 
    $$\gamma-\delta-K(d/2-1)\ge -\varepsilon(d/2-1)(2\gamma-\delta)+4\gamma-2\gamma^2-2\delta+\delta\gamma-1.$$
    That is,
    \begin{align}\label{K.small}
        K(d/2-1) \le \varepsilon(d/2-1)(2\gamma-\delta)+(\gamma-2)(2\gamma-\delta)+1+\gamma-\delta.
    \end{align}
   Our job is reduced to verifying that given $m\in \mathbb N$, $d>3$, (as well as $\gamma$ and $\delta$) there is some $K>\frac{\gamma-\delta}{d/2-1}$  (thus depending on $\gamma$ and $\delta$,  but being uniform in $d>d_0(\gamma,\delta)$),  such that 
     \eqref{K.small} holds.
    Putting things together, $K$ must satisfy that
    $$
    L:= \frac{\gamma-\delta}{d/2-1} < K < \varepsilon(2\gamma-\delta) + \frac{(\gamma -2)(2\gamma-\delta)+1+\gamma-\delta}{d/2-1}=:U.
     $$
   Keeping in mind that $\delta<1$,  write
    $$U= \varepsilon(2\gamma-1) + (1-\delta)\varepsilon+\frac{(\gamma -2)(2\gamma-\delta)+1+\gamma-\delta}{d/2-1}.$$
    Recall also, that  $\varepsilon=\varepsilon(\gamma,\delta)$ is guaranteed to exists by Lemma \ref{lem:constantincrdiam} and \emph {it does not depend on} $d$. Hence, with $\gamma,\delta$ (and thus also $\varepsilon$) fixed, we may pick a $d^*_0=d^*_0(\gamma,\delta)$ such that for $d>d^*_0$,
    $U>\varepsilon(2\gamma-1).$
    So the sought $K$ exists if $d>d^*_0(\gamma,\delta)$ as well as
    $$\frac{\gamma-\delta}{d/2-1} < \varepsilon(2\gamma-1) \iff d>\frac{2(\gamma-\delta)}{\varepsilon(2\gamma-1)}+2=:d^{**}_0.$$
    Thus,  $d_0:=\max\{d^*_0, d^{**}_0\}$ satisfies the requirements and the lemma is proven. WE ALSO HAVE TO CHECK THE POWER OF 2 IN \eqref{long.bound}!! I rewrote the whole computation. I check the whole thing together and not separately the powers of n and 2. It works, provided $d\ge 3$. So far it is only on paper, still have to type it up.
    




==> generalized-PA.tex <==
\section{Random Preferential Attachment Trees}

Let $\{Z_n\}_{n\geq 1}$ be a sequence of independent positive integer random variables satisfying 
$\mathbb{P}(1\leq Z_n<+\infty)=1$, for all $n$.  As we shall soon seen, this sequence encodes the growth in our random graph model, specifically the (random) number of new vertices added at every time $n$.  

\medskip 
Let $T_0=(V_0, E_0)$ be a finite (initial) tree and denote $m_0=|V_0|$ the initial number of vertices. The {\em Random  Preferential Attachment Tree (RPAT)} we consider here, is defined as follows: at every time $n\geq 1$ a random number of vertices (leaves) $Z_n$ is generated and, conditioned on the random tree at time $n-1$, i.e.,  $T_{n-1}=(V_{n-1}, E_{n-1})$,  all the $Z_n$ new leaves  are attached, through $Z_n$ edges, to a unique vertex in $V_{n-1}$ chosen according to preferential attachment; specifically,  a vertex $v \in V_{n-1}$ is chosen with probability proportional to $\degree{T_{n-1}}{v}$ (linear preferential attachment). 


The number of vertices at time $n$, is a random variable given by \[
m_n:=|V_n|= m_0 + \sum_{i=1}^n Z_i\;,
\]
and its expectation $\mathbb{E}(m_n)=:M_n= m_0 + \sum_{i=1}^n \mathbb{E}(Z_i)$. 


We are interested in the degree distribution of the graph generated by RPAT. Without loss of generality, we shall assume that $T_0$ is a single vertex $r$ with a self-loop, thus $m_0=1$ and $\degree{T_0}{r}=2$. Let  $\{\mathcal{F}_n\}_{n\geq 1}$ denote the natural filtration generated by the RPAT process, and  let us denote by $N_n(k)$ the number of vertices of degree $k$ ($k\geq 1$) at time $n$. The following recurrence holds: for $k=1$,
\begin{align*}
\mathbb{E}\left(N_n(1) \mid \mathcal{F}_{n-1}, Z_n \right)& = Z_n + N_{n-1}(1)\left( 1- \frac{1}{2m_{n-1}}\right) \;,
\end{align*}
and for $k\geq 2$, 
\begin{align*}
    \mathbb{E}&\left(N_n(k) \mid \mathcal{F}_{n-1},Z_n \right) = \sum_{i=1}^{\infty}  \mathbb{E}\left(N_n(k) \mid \mathcal{F}_{n-1}, Z_n=i \right)\mathbb{1}\{Z_n=i\} \\
&= \frac{1}{2m_{n-1}}\sum_{i=1}^{k-1} (k-i) N_{n-1}(k-i) \mathbb{1}\{Z_n=i\} +   N_{n-1}(k) \left( 1- \frac{k}{2m_{n-1}} \right) 
\\
&= \sum_{\ell = 1}^{k-1} \ell \frac{N_{n-1}(\ell)}{2m_{n-1}} \mathbb{1}\{Z_n= k-\ell\}  +   N_{n-1}(k) \left( 1- \frac{k}{2m_{n-1}} \right) \;,
\end{align*}
since 
\[
\mathbb{E}\left(N_n(k) \mid \mathcal{F}_{n-1}, Z_n=i \right) = \mathbb{1}\{i<k\}  N_{n-1}(k-i) \left( \frac{k-i}{2m_{n-1}-1} \right) +  N_{n-1}(k) \left( 1- \frac{k}{2m_{n-1}} \right) \;.
\]
 Taking expectation on both sides (using independence between $Z_n$ and $\mathcal{F}_{n-1}$) we obtain
\begin{align*}
 \mathbb{E}\left(N_n(1)\right)& = \mathbb{E}\left(Z_n\right) + \mathbb{E}\left(N_{n-1}(1)\left(1-\frac{1}{2m_{n-1}} \right)\right)\;, \qquad k=1\;,
 \\
 \mathbb{E}\left(N_n(k)\right) &= \sum_{\ell =1}^{k-1} \ell\, \mathbb{E} \left( \frac{N_{n-1}(\ell)}{2m_{n-1}} \right) \mathbb{P}(Z_n= k-\ell)+ \mathbb{E} \left( N_{n-1}(k)\left(1- \frac{k}{2m_{n-1}}\right) \right) \;, \qquad k\geq 2\;.
\end{align*}


\com{
Under which assumptions we have that for every fixed $k$ and every $n$ 
\[
\left\vert \mathbb{E}\left(\frac{N_n(k)}{2m_n}\right) - \frac{\mathbb{E}\left(N_n(k)\right)}{\mathbb{E}(2m_n)}  \right\vert\leq o_n(1) ?
\]
}

Assuming the above assumption holds, the recurrence becomes 
\begin{align*}
 \mathbb{E}\left(N_n(1)\right)& = \mathbb{E}\left(Z_n\right) + \mathbb{E}\left(N_{n-1}(1) \right)\left(1-\frac{1}{2M_{n-1}} \right) + o_n(1)\;, \qquad k=1\;,
 \\
 \mathbb{E}\left(N_n(k)\right) &= \sum_{\ell =1}^{k-1} \ell\,  \frac{\mathbb{E}\left(N_{n-1}(\ell)\right)}{2M_{n-1}} \mathbb{P}(Z_n= k-\ell)+ \mathbb{E} \left( N_{n-1}(k)\right) \left(1- \frac{k}{2M_{n-1}} \right) {\color{red}+ o_n(1)} \;, \qquad k\geq 2\;.
\end{align*}

\com{To be able to apply the Lemma in Chung, we need to assume:
\begin{align*}
&\lim_{n \to +\infty} \frac{n}{2M_n} = C \in (0, + \infty), \quad i.e., M_n = \Theta(n)\;
\\
&\lim_{n \to +\infty} \mathbb{E(Z_n)}= c\;
\end{align*}
These assumption would imply \[
\lim_{n \to +\infty}\frac{\mathbb{E}\left(N_n(1)\right)}{n} = \frac{c}{1+C}\;.
\]
Then, for $k=2$, we would have
\[
\mathbb{E}\left(N_n(2)\right) =  \frac{\mathbb{E}\left(N_{n-1}(1)\right)}{2M_{n-1}} \mathbb{P}(Z_n= 1)+ \mathbb{E} \left( N_{n-1}(2)\right) \left(1- \frac{2}{2M_{n-1}} \right) {\color{red}+ o_n(1)} \;,
\]
so we would also need something like 
\[
\lim_{n \to +\infty} \frac{n}{2M_n} \mathbb{P}(Z_n=1) = \widetilde{C} \in (0, + \infty)
\]
to infer that
\[
\lim_{n \to +\infty}\frac{\mathbb{E}\left(N_n(2)\right)}{n} = \frac{\widetilde{c}}{1+C}\frac{\widetilde{C}}{1+2C}\;.
\]
}

==> no_power_law_example.tex <==
In order to illustrate that for the \name random walk recurrence is not equivalent to observing a scale-free tree sequence, we provide an example of a sequence $\{Z_n\}_{n\ge 1}$ under which the walker is recurrent but the corresponding tree sequence has a limiting degree distribution which is very different from the power-law. In fact, we prove that in this setup, the proportion of leaves converges to one almost surely. 


To carry out this program, for a fixed $\delta >0$, consider the sequence of real numbers $(p_n^\delta)_{n \ge 1}$, with $p_n^{(\delta)} := {n^{-\delta}}$, 
and the laws 
\begin{equation}\label{def:zn}
L^{(\delta)}_n:= 
\begin{cases}
\log n,\text{ with probability }p_n^{(\delta)};\\
0,\text{ with probability }1-p_n^{(\delta)}.
\end{cases}
\end{equation}
Regarding the $\mathcal{L}^{(\delta)}$-\name process  we have the following result:
\begin{proposition}[Recurrence with leaves only]\label{prop:deltadist} For the $\mathcal{L}^{(\delta)}$-\name process satisfying \eqref{def:zn}, the random walk is recurrent for all $\delta \in (2/3,1]$. Furthermore, if $N_n(1)$  denotes the number of leaves and $|\mathcal{V}_n|$ the total number of vertices in $T_n$, then
$$
    \lim_{n\to \infty } \frac{N_n(1)}{|\mathcal{V}_n|} = 1\;, \quad  \mathbb{P}_{T_0,x;\mathcal{L}^{(\delta)}}\text{-a.s.}
$$
\end{proposition}
\underline{Intuition:} By \eqref{def:zn}, when the walker adds new leaves at time $n$, it adds an amount of $\log n$. Heuristically, Proposition~\ref{prop:deltadist} says that this quantity is not large enough to ``trap'' the walker in some neighborhood of a vertex, so the walk is still recurrent. Nonetheless, it is large enough to change the power-law degree distribution dramatically, producing trees whose empirical degree distribution converges to the degenerate distribution over $\mathbb{N}$ which puts all the mass at $1$.
\begin{proof}[Proof of Proposition \ref{prop:deltadist}]
We check recurrence first.

\underline{Recurrence of the walk.}  By Theorem \ref{thm:general_recurrence}, we need to show that $\{Z^{(\delta)}_n\}_n$ satisfies all the assumptions (A1)-(A3) of that theorem. Assumptions (A1) and (A2) trivially follow  from the definitions of $p_n^{(\delta)}$ and $Z^{(\delta)}_n$. For (A3), recalling that $\delta \in (2/3,1]$, use that
$
    E(Z^{(\delta)}_n) = \frac{\log n}{n^{\delta}},$
    yielding $$M_n = \sum_{k=1}^n \frac{\log k}{k^{\delta}} \le  \log n \sum_{k=1}^n \frac{1}{k^{\delta}}\le \log n\int_0^n x^{-\delta}\, dx=(1-\delta)^{-1}\log n \cdot n^{1-\delta} \;,
$$
hence $$(1-q_n)\cdot M_n^2\le {n^{-\delta}}\cdot(1-\delta)^{-2} n^{2-2\delta}(\log n)^2=
 (1-\delta)^{-2}n^{2-3\delta}(\log n)^2\to 0\;,$$ since $\delta>2/3.$ This proves recurrence. \\


Next we check the degree distribution.

\underline{Proportion of leaves.} Define the stopping times
\begin{equation}\label{eq:stopping.t}
     \tau_0\equiv 0;\qquad  \tau_k: = \inf \{ n > \tau_{k-1} \; : \; Z^{(\delta)}_n = \log n \}\;,\qquad k\ge 1\;.
\end{equation}
 Since $\delta \le 1$, it follows that all the $\tau_k$ are finite $P$-a.s. Introduce the shorthands 
$$
\widetilde{N}_k := N_{\tau_k}(1); \quad \widetilde{V}_k := |\mathcal{V}_{\tau_k}|\;.
$$
By \eqref{eq:stopping.t}, we have that
$
\widetilde{V}_k = |\mathcal{V}_0| + \sum_{j=1}^k \log(\tau_k)
$ where $|\mathcal{V}_0|$ is size of the initial tree $T_0$. Moreover, observe that whenever a certain amount of new leaves is added, even in the ``worst case scenario'' when new vertices are added to a leaf, only one leaf has to be subtracted from the total number of leaves. This implies that 
\begin{equation*}
    \widetilde{N}_k \ge \sum_{j=1}^k\log(\tau_j) -k = \widetilde{V}_k - |\mathcal{V}_0| - k\;,  \quad
    \mathbb{P}_{T_0,x;\mathcal{L}^{(\delta)}}\text{-a.s.}
    % \mathbb{P}_{x_0,T_0, Z^{(\delta)}}\text{-a.s.}\;.
\end{equation*}
Using that $\tau_k \ge k$ almost surely, we have that 
\[
\widetilde{V}_k \ge \sum_{j=1}^k \log j \ge \int_1^k \log x\, dx= k(\log k-1)+1\;,
\]
yielding that
\begin{align*}
 &\frac{\widetilde{N}_k}{\widetilde{V}_k} \ge 1 - \frac{ (|\mathcal{V}_0| + k)}{\widetilde{V}_k}\ge 1- \frac{ (|\mathcal{V}_0| + k)}{k(\log k-1)+1}\\
 &\implies \liminf_{k \to \infty} \frac{\widetilde{N}_k}{\widetilde{V}_k} \ge 1\;,
 \quad
 \mathbb{P}_{T_0,x;\mathcal{L}^{(\delta)}}\text{-a.s.}\;
%  \mathbb{P}_{x_0,T_0, Z^{(\delta)}}\text{-a.s.}\;.
\end{align*}
To conclude the proof use that $\widetilde{N}_k \le \widetilde{V}_k$ along with the obvious fact that the sequence $\{N_n(1)/|\mathcal{V}_n|\}_n$ only changes its values at the stopping times $\tau_k$'s.
\end{proof}

==> recurrence.tex <==
In this section we  prove Theorem~\ref{thm:general_recurrence}, which states that the under certain assumptions on $\{Z_n\}_{n\geq 1}$ the random walk is recurrent. Without the loss of generality, throughout this section we may and will assume that our initial tree $T_0$ consists of just a single vertex, denoted by  $o$.  As will become clear along the proof, the initial tree plays no important role in the long-time behavior of the walker.

\medskip 
%\underline{Filtrations:} 
%Recall that $Z_n\sim L_n$ is the number of leaves added at time $n$. We will write $\{\mathcal{F}_n\}_{n\ge 1}$ for the natural filtration for the  $\mathcal{L}$-\name process, whereas $\{\mathcal{G}_n\}_{n\ge 1}$ will denote the natural filtration for $\{Z_n\}_{n \ge 1}$ only. 

\begin{proof}[Proof of Theorem~\ref{thm:general_recurrence}] We begin noticing that by (A3), we can choose a sequence $g_n$ such that
    \begin{equation*}
        g_n \to \infty \text{ and } (1-q_n)\cdot g_n \cdot M_n^2 \to 0, \text{ as }n \to \infty\;.
    \end{equation*}
Also consider the following random variable
\begin{equation*}
    W_n = \sum_{k=n}^{n+g_nM_n^2} \mathbb{1}\{ Z_k \ge 1\}\;.
\end{equation*}
In words, $W_n$ counts how many times the walker has added at least one leaf during the time interval $[n, n+g_nM_n^2]$. By (A2), it follows that 
\begin{equation}\label{eq:mean}
    \Ed_{T_0, x ; \mathcal{L}}\left[W_n\right] = \sum_{k=n}^{n+g_nM_n^2} 1-q_k \le (1-q_{n})\cdot g_n \cdot M_n^2 \to 0\;,
\end{equation}
as $n$ goes to infinity. Now, let $A_n$ denote the following event
\begin{equation*}
    A_n = \{ \text{no grow in the interval }[n, n+g_nM_n^2]\}\;,
\end{equation*}
that is, the walker did not add any new leaves to the tree in the time interval $[n, n+g_nM_n^2]$.
By the bound in \eqref{eq:mean} and Markov Inequality we have that
\begin{equation}\label{eq:an}
    \Pd_{T_0, x; \mathcal{L}}(A_n^c) = \Pd_{T_0, x; \mathcal{L}}(W_n \ge 1) \le \Ed_{T_0, x; \mathcal{L}}\left[W_n\right] = o(1)\;.
\end{equation}
Finally, let $B_n$ denote the following event
\begin{equation*}
    B_n := \{ X \text{ visits the root some time in }[n, n+g_nM_n^2]\}\;.
\end{equation*}
Using the fact (see \cite{brightwellwinkler1990}) that the cover time of a tree of size $k$ is at most $2k^2$ gives us 
\begin{equation}\label{eq:bnan}
    \Pd_{T_0, x; \mathcal{L}}(B_n^c, A_n | V_n \le g_n^{1/4}M_n) \le \frac{\sqrt{g_n}M_n^2}{g_n M_n^2} = o(1)\;.
\end{equation}
By the simple Markov property we have that on the event $A_n$, $\{X_k\}_n^{n + g_nM_n^2}$ is distributed as a SSRW on $T_n$, which is a tree with at most $g_n^{1/4}M_n$ vertices. And $B_n^c$ means that this SRRW did not cover the entire graph in $g_n M_n^2$ steps. The bound then follows by Markov Inequality. Finally, 
\begin{equation*}
    \begin{split}
        \Pd_{T_0, x; \mathcal{L}}(B_n^c) & \le  \Pd_{T_0, x; \mathcal{L}}(B_n^c, A_n, V_n \le g_n^{1/4}M_n) + \Pd_{T_0, x; \mathcal{L}}(A_n^c) + \Pd_{T_0, x; \mathcal{L}}(V_n \ge g_n^{1/4}M_n) = o(1)\;,
    \end{split}
\end{equation*}
since the first term at the RHS is $o(1)$ by \eqref{eq:bnan}, the second one is $o(1)$ by \eqref{eq:an}, whereas the third one is $o(1)$ by Markov Inequality. The above inequality yields
$$
    \Pd_{T_0, x; \mathcal{L}}(X \text{ visits the root some time in }[n, n+g_nM_n^2]) = P(B_n) = 1-o(1)\;.
$$
Finally, by Fatou's Lemma
$$
\Pd_{T_0, x; \mathcal{L}}(\limsup_{n\to \infty} B_n ) \ge \limsup_{n\to \infty}\Pd_{T_0, x; \mathcal{L}}(B_n) = 1\;,
$$
which proves that the root is visited infinitely many times for any initial condition $(T_0,x)$. To extend the result to a vertex which is eventually added to the tree, we apply Strong Markov Property to the Markov process $\{(T_n,X_n)\}_{n\in \mathbb{N}}$ together with the result for a fixed initial condition. This proves that even those vertices which are added by the process in the future are visited i.o.
\end{proof}





==> transience.tex <==


In this section we  prove Theorem~\ref{thm:transient}, which states that the random walk in  $p_n$-\name with $p_n=\Theta(n^{-\gamma})$ is transient  for $\gamma \in (0,1/4)$. 


Consider the following sequence of stopping times: $\eta_0\equiv 0$, and for every $k\geq 1$
\[
\eta_k := \inf\{n> \eta_{k-1}: \degree{T_n}{X_{n}}\geq 2 \}\;, 
\] 
i.e., the times at which  the random walk resides on a vertex of degree greater or equal to $2$ (right before the tree structure is modified). The stopping times $\eta_k$'s are finite $\Pd_{o, T_0, Z}$-almost surely, for every $k$.  As a matter of fact, let  $\Delta\eta_k= \eta_{k}-\eta_{k-1}$ denote the time interval between two consecutive stopping times;  for $\Delta\eta_k$ to be bigger that $m$, it must be the case that  for $m$ consecutive steps after time $\eta_{k-1}$,  the random walk  steps into a leaf (vertex of degree one).  Thus,  we obtain that for every $m\geq 2$, 
\[
\Pd_{o, T_0, Z}(\Delta\eta_k \geq  m \mid \mathcal{F}_{\eta_{k-1}})\leq  \prod_{j=2}^m \frac{1}{2(\eta_{k-1}+ j)^{\gamma}}\leq k^{-(m-1) \gamma}\;,
\]
 where, in the last inequality we used that $\eta_{k-1}\geq k-1$, for all realizations. 
%
Averaging out with respect to $\mathcal{F}_{\eta_{k-1}}$, we obtain 
\begin{align}\label{eq:Delta-eta}
\Pd_{o, T_0, Z}(\Delta\eta_k \geq  m)\leq k^{-(m-1) \gamma}\;.
\end{align}
 
\com{
Hence, for any fixed  $\gamma$, if $(m-1)\gamma > 1$,  by Borel-Cantelli 
$\sum_{k=1}^\infty \mathbb{1}\{\Delta\eta_k \geq  m\}<+\infty$,  $\Pd_{o, T_0, Z}$-almost surely. \texttt{THIS  should impliy that $N_n\ to +\infty$ almost surely}}


\bigskip 
\com{
 %
 Moreover, TO BE FIXED
\begin{align}\label{eq:eta}
\Pd_{o, T_0, Z}\left( \eta_n \geq  m n \right)\leq \Pd_{o, T_0, Z}\left(\bigcup_{j=1}^n \{\Delta \eta_j \geq m\} \right)\leq \sum_{j=1}^n j^{-(m-1)\gamma}= C n^{1-(m-1)\gamma}\;,
\end{align}
where, $C$ is a positive constant depending on $\gamma$ and $m$ only. 
Hence, if $(m-1)\gamma >2$,  by Borel-Cantelli we have that $\eta_n\geq m n$ only a finite number of times and $\lim_{n\to \infty}\mathbb{1}\{\eta_n<mn\}=1$,  $\Pd_{o, T_0, Z}$-almost surely. FIX THE CONSTANT C}

%
Since $\eta_k$'s are finite $\Pd_{o, T_0, Z}$-almost surely, the sequence of random variable $\{Z_{\eta_k+1}\}_{k \geq 0}$ is well defined. Despite the stopping time $\eta_k$ depends on the overall process up to that time,   the random variables $\{Z_{\eta_k+1}\}_{k \geq 0}$ are independent, as a consequence of the independence of the original random variables  $\{Z_n\}_{n\geq 0}$.

As it will become clear from the proof of Theorem~\ref{thm:transient}, an important step  is to lower bound the following quantity
\[
L_n:=\sum_{j=1}^n Z_{j+1}Z_{j}\mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}\geq 2\right\} \;. 
\]
A lower bound on $L_n$  is provided in the next lemma. 

\begin{lemma}\label{lem:L_n}
For every $m$ fixed and  $n$ sufficiently large, the following bound holds $\Pd_{o, T_0, Z}$-almost surely
\begin{align}\label{eq:Ln}
\mathbb{1}\left\{ \eta_{\lfloor n/m \rfloor} < n \right\} L_n &\geq \mathbb{1}\left\{ \eta_{\lfloor n/m \rfloor} < n \right\} \left( \sum_{j=1}^{\lfloor n/m \rfloor} \Ed_{o, T_0, Z}[\widehat{Z}_j]   
- \sqrt{2 n \log \log n}\right)\;.
%
%\quad \text{$\Pd_{o, T_0, Z}$-almost surely}\;,
%\mathbb{1}\left\{ \eta_{\lfloor n/m \rfloor} < n \right\} |L_n| &\geq \mathbb{1}\left\{ \eta_{\lfloor n/m \rfloor} < n \right\} \left( \sum_{j=1}^{\lfloor n/m \rfloor} g_j   
%- \sqrt{2 \sum_{j=1}^{\lfloor n/m \rfloor} g_j \log \log \sum_{j=1}^{\lfloor n/m \rfloor} g_j}\right)\;,
%%\quad \text{$\Pd_{o, T_0, Z}$-almost surely}\;,
\end{align}
%	where, $g_j = \Ed_{o, T_0, Z}[\widehat{Z}_j]$. \com{we could also put $\sqrt{n\log \log n}$ in the remainder term}
\end{lemma}

\com{The RHS in \eqref{eq:Ln} should be corrected accordingly...}
\begin{proof}
Due to the difinition of $L_n$, for every $m<n$,  the following bound holds (for all realizations)
\[
\mathbb{1}\left\{ \eta_{\lfloor n/m \rfloor} < n \right\}L_n \geq  \mathbb{1}\left\{ \eta_{\lfloor n/m \rfloor} < n \right\}\sum_{k=1}^{\lfloor n/m \rfloor} Z_{\eta_k + 2}Z_{\eta_k + 1}\geq \mathbb{1}\left\{ \eta_{\lfloor n/m \rfloor} < n \right\} \sum_{k=1}^{\lfloor n/2m \rfloor} Z_{\eta_{2k} + 2}Z_{\eta_{2k} + 1}
\;.
\]
Note that $\{Z_{\eta_{2k} + 1}\}_{k\geq 0}$ and $\{Z_{\eta_{2k} + 2}\}_{k\geq 0}$ are independent, while this is not necessarily the case for $\{Z_{\eta_{k} + 1}\}_{k\geq 0}$ and $\{Z_{\eta_{k} + 2}\}_{k\geq 0}$; this is the reason why we consider the last inequality above. 
Thus, it is enough to show that $\sum_{k=1}^{\lfloor n/2m \rfloor} Z_{\eta_{2k} + 2}Z_{\eta_{2k} + 1}$  is greater or equal to the factor on the RHS in Equation~\eqref{eq:Ln}.  

\medskip 
\com{From here the proof should be adapted.....}
Let us consider  the sequence of independent and  centered random variables  $Y_k = \Ed_{o, T_0, Z}[\widehat{Z}_k] - \widehat{Z}_k$, and denote by $\sigma_k^2= \Ed_{o,T_0,Z}[Y_k^2]$. Setting  
$S_n=\sum_{k=1}^n Y_k$ and $s_n^2=\sum_{k=1}^n\sigma_k^2$, since 
$|Y_n|= o \left( \frac{s_n}{\sqrt{\log \log s_n}} \right)$, for every $n$ \com{check!!}, we can apply the Law of the Iterated Logarithm  of Kolmogorov to obtain that
\[
\limsup_{n \to \infty} \frac{S_n}{\sqrt{2s^2_n\log \log s^2_n}}=1\;, \quad \text{$\Pd_{o, T_0, Z}$-almost surely}\;.
\]
Thus, there exists $n_0$, such that for all $n\geq n_0$, $S_n \leq \sqrt{2s^2_n\log \log s^2_n}$; thus we obtain that 
From the latter, we obtain that
\begin{align*}
\sum_{k=1}^n \Ed_{o, T_0, Z}[\widehat{Z}_k] - \sum_{k=1}^n \widehat{Z}_k \leq \sqrt{2s^2_n\log \log s^2_n}  
\;,
\end{align*}
$\Pd_{o, T_0, Z}$-almost surely. Since  $m$ is fixed, and using that  $s^2_n\leq \sum_{k=1}^n \Ed_{o, T_0, Z}[\widehat{Z}_k]\leq n$, the claim follows. 
%Due to the difinition of $L_n$, for every $m<n$,  the following bound holds (for all realizations)
%\[
%|L_n| \geq \sum_{k=1}^n\widehat{Z}_k \mathbb{1}\left\{ \eta_k < n \right\}\geq \sum_{j=1}^{\lfloor n/m \rfloor} \widehat{Z}_j \mathbb{1}\left\{ \eta_j < jm \right\} \geq \sum_{j=1}^{\lfloor n/m \rfloor} \widehat{Z}_j \mathbb{1}\left\{ \Delta\eta_j < m \right\}
%\;.
%\]
%Thus, it is enough to show that $\sum_{j=1}^{\lfloor n/m \rfloor} \widehat{Z}_j \mathbb{1}\left\{ \Delta\eta_j < m \right\}$  is greater or equal to the RHS in Equation~\eqref{eq:Ln}.  
%
%Let us begin noticing that  $\widehat{Z}_j$ is independent of $\mathbb{1}\left\{ \Delta\eta_j \leq m \right\}$, for all $j$ \com{check}. Moreover, also $\widehat{Z}_j \mathbb{1}\left\{ \Delta\eta_j < m \right\}$ are independent \com{across $j$ check!!}. 
%
% 
%Let us consider  the sequence of centered random variables  $Y_k = \left(p_{\eta_k+1} - \widehat{Z}_k\right) \mathbb{1}\left\{ \Delta\eta_k < m \right\}$ \com{CHeck Independence....}, and denote by $\sigma_k^2= \Ed_{o,T_0,Z}[Y_k^2]$. Setting  
%$S_n=\sum_{k=1}^n Y_k$ and $s_n^2=\sum_{k=1}^n\sigma_k^2$, since 
%$|Y_n|= o \left( \frac{s_n}{\sqrt{\log \log s_n}} \right)$, for every $n$ \com{check!!}, we can apply the Law of the Iterated Logarithm  of Kolmogorov to obtain that
%\[
%\limsup_{n \to \infty} \frac{S_n}{\sqrt{2s^2_n\log \log s^2_n}}=1\;, \quad \text{$\Pd_{o, T_0, Z}$-almost surely}\;.
%\]
%Thus, there exists $n_0$, such that for all $n\geq n_0$, $S_n \leq \sqrt{2s^2_n\log \log s^2_n}$, $\Pd_{o, T_0, Z}$-almost surely. 
%From the latter, we obtain 
%\begin{align*}
%\sum_{k=1}^n p_{\eta_k+1}\mathbb{1}\left\{ \Delta\eta_k < m \right\} - \sum_{k=1}^n \widehat{Z}_k\mathbb{1}\left\{ \Delta\eta_k < m \right\} \leq \sqrt{2s^2_n\log \log s^2_n}  
%\;. 
%\end{align*}
%Given that $m$ is fixed, and using that  $s^2_n\leq \sum_{k=1}^n p_{\eta_k+1}\Pd_{o, T_0, Z}(\Delta\eta_k <  m)$, the claim follows. 
\end{proof}


The next lemma tells us that if $m$ is sufficiently large with respect to $\gamma$, i.e., $(m-1)\gamma>1$,  the two partial sums $\sum_{k=1}^n p_k p_{k+1}$ and $\sum_{k=1}^{\lfloor n/2m \rfloor} \Ed_{o, T_0, Z}[Z_{\eta_{2k} + 2}Z_{\eta_{2k} + 1} ]$ are asymptotically in $n$ of the same order. 

\com{The next lemma should also be modified accordingly...}

\com{think whether we use some bound on $\gamma$ in the next lemma!}
\begin{lemma}\label{lem:two-sums}
For every $\gamma$ and for every $m$ fixed  such that $(m-1)\gamma>1$,   asymtotically in $n$, it holds that 
\[
\sum_{k=1}^{\lfloor n/m \rfloor} \Ed_{o, T_0, Z}[\widehat{Z}_k] = \Theta \left( \sum_{k=1}^n p_{k} \right)\;.
\]
\end{lemma}

\begin{proof}
Let us begin observing that
\begin{align*}
\Ed_{o, T_0, Z}[\widehat{Z}_k]= \Ed_{o, T_0, Z}[Z_{\eta_k +1}]= \sum_{j =k}^\infty p_{j + 1}\Pd_{o, T_0, Z}(\eta_k = j)
\leq p_k
\;,
\end{align*}
where, we used the monotonicity of $(p_n)_{n\geq 0}$. Thus,  $\sum_{k=1}^{\lfloor n/m \rfloor} \Ed_{o, T_0, Z}[\widehat{Z}_k] \leq \sum_{k=1}^n p_{k}$, for every $m$. 
We are left with showing that,  for  sufficiently large $n$,  there exists a constant $c$ such that $\sum_{k=1}^n p_k \leq c \sum_{k=1}^{\lfloor n/m \rfloor} \Ed_{o, T_0, Z}[\widehat{Z}_k]$.
%
For every $m\geq 2$ it holds that 
\begin{align*}
&\Ed_{o, T_0, Z}[\widehat{Z}_k]= \Ed_{o, T_0, Z}[Z_{\eta_k +1}]= \sum_{j =k}^\infty p_{j + 1}\Pd_{o, T_0, Z}(\eta_k = j)\geq p_{mk}\Pd_{o, T_0, Z}(\eta_k \leq m k)\;.
%%= \sum_{j =k}^\infty (j + 1)^{-\gamma}\Pd_{o, T_0, Z}(\eta_k = j)
%\\
%&= \sum_{\ell =1}^{\infty}\sum_{j=(\ell-1)m}^{\ell m -1} p_{k+j+1}\Pd_{o, T_0, Z}(\eta_k = k+j)\geq \sum_{\ell =1}^{\infty}p_{k+\ell m} \Pd_{o, T_0, Z}((\ell-1)m\leq \eta_k - k \leq \ell m -1 )  
\end{align*}
 Note that, for $m$ such that  $(m-1)\gamma>1$, by Equation~\eqref{eq:eta}, we know that for any $\varepsilon>0$, there exists a $k_0$ such that
 $\Pd_{o, T_0, Z}(\eta_k \leq m k)>(1-\varepsilon)$,   for every  $k\geq k_0$.  Therefore, for $n$ sufficiently large,  
\begin{align*}
\sum_{k=1}^{\lfloor n/m \rfloor} \Ed_{o, T_0, Z}[\widehat{Z}_k]&\geq  \sum_{k=1}^{k_0-1} p_{mk}\Pd_{o, T_0, Z}(\eta_k \leq m k)  + (1-\varepsilon) \sum_{k=k_0}^{\lfloor n/m \rfloor} p_{mk}
\\
&\geq C + \frac{1-\varepsilon}{m}\sum_{\ell = mk_0}^n p_\ell=  C - \frac{1-\varepsilon}{m}\sum_{\ell = 1 }^{mk_0-1}p_\ell  + \frac{1-\varepsilon}{m}\sum_{\ell = 1}^n p_\ell \;,
\end{align*}
and the claim follows.  \com{Here we only need that $\Pd_{o, T_0, Z}(\eta_k \leq m k)\to 1$, not almost sure covergence?} 
\end{proof}

\com{Up to now we did not use $\gamma < 1/2$!}





We are now ready to prove Theorem~\ref{thm:transient}. 


% \begin{theorem}[Transient regime]\label{thm:transient}
% The random walk in $p_n$-\name with $p_n=\Theta(n^{-\gamma})$ is transient, for every $\gamma \in (0,1/2)$. 
% \end{theorem}
\begin{proof}[Proof of Theorem~\ref{thm:transient}]
Let $d_n={\rm dist}_{T_n}(X_n, X_0)$ denote the graph distance between  $X_n$ and $X_0$ in the tree $T_n$ (i.e., at time $n$). We are going to show that, for every $\gamma \in (0,1/2)$, there exists a positive constant $c$ \com{independent of $\gamma$?} such that 
\begin{align}\label{eq:limsup}
\liminf_{n\to \infty} \frac{d_n}{n^{1-2\gamma}} \geq c \;, \quad  \text{$\Pd_{o, T_0, Z}$-almost surely}\;. 
\end{align}


Let $\Delta d_n:= d_n -d_{n-1}$ denote the distance increment at time $n$ ($d_0 \equiv 0$). Let us decompose $d_n$ as follows:
\begin{equation}\label{eq:decom}
\begin{split}
d_n = \sum_{j=1}^n \Delta d_j = \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}=1\right\} + \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq 2\right\}\;.
\end{split}   
\end{equation}
%\begin{equation}
%\begin{split}
%d_n = \sum_{j=1}^n \Delta d_j &= \underbrace{\sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}=1\right\}}_{A_n(1)} \Big( \mathbb{1}\left\{Z_{j+1}=1\right\} + \mathbb{1}\left\{Z_{j+1}=0\right\}\Big) 
%\\
%& + \underbrace{\sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}=2\right\}}_{A_n(2)} \Big( \mathbb{1}\left\{Z_{j+1}=1\right\} + \mathbb{1}\left\{Z_{j+1}=0\right\}\Big)
%\\
%& + \underbrace{\sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq 3\right\}}_{A_n(3)} \Big( \mathbb{1}\left\{Z_{j+1}=1\right\} + \mathbb{1}\left\{Z_{j+1}=0\right\}\Big)\;.
%\end{split}   
%\end{equation}

\begin{claim}{} The following bound holds deterministically 
	\begin{equation*}
	\begin{split}
& \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}=1\right\} + \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq 2\right\} \mathbb{1}\left\{\degree{T_{j+1}}{X_{j}}=1\right\}  \geq -1 
% \\
% & \geq \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq 2\right\} \mathbb{1}\left\{\degree{T_{j+1}}{X_{j}}\geq 2\right\}  \mathbb{1}\left\{Z_{j+1}=0\right\}
\;.
\end{split}
	\end{equation*}
\end{claim}
\begin{claimproof}
% \com{Maybe we could be more formal proceeding by induction...}
Note that   $\mathbb{1}\left\{\degree{T_{j+1}}{X_{j}}=1\right\}=1$ implies $\mathbb{1}\left\{\degree{T_{j}}{X_{j-1}}\geq 2\right\}=1$, as wells as  $\Delta d_{j+1}=-1$ e $\Delta d_{j}=1$. \com{intuition in words if deemed necessary}. 
Thus, 
	\begin{equation*}
	\begin{split}
& \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}=1\right\} + \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq 2\right\} \mathbb{1}\left\{\degree{T_{j+1}}{X_{j}}=1\right\} 
\\
&= \Delta d_1 \mathbb{1}\left\{\degree{T_1}{X_{0}}=1\right\} + 
\sum_{j =1}^{n-1} \left( \Delta d_{j+1}  + \Delta d_{j} \right)\mathbb{1}\left\{\degree{T_{j+1}}{X_{j}}=1\right\} 
\\
& \qquad + \Delta d_n \mathbb{1}\left\{\degree{T_{n+1}}{X_{n}}=1\right\} \geq -1 + \Delta d_n \mathbb{1}\left\{\degree{T_{n+1}}{X_{n}}=1\right\}   
\;.
\end{split}
	\end{equation*}
\end{claimproof}

From Equation~\ref{eq:decom} and using the above claim,  we obtain that 
\begin{equation*}
\begin{split}
d_n &\geq \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq 2\right\}\mathbb{1}\left\{\degree{T_{j+1}}{X_{j}}\geq 2\right\}
\left( \mathbb{1}\left\{Z_{j+1}=1\right\} + \mathbb{1}\left\{Z_{j+1}=0\right\}  \right) 
\\
&
=\underbrace{\sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq  2\right\}\mathbb{1}\left\{Z_{j+1}=1\right\} }_{A_n}
\\
& \quad + \underbrace{\sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq 2\right\}\mathbb{1}\left\{\degree{T_{j+1}}{X_{j}}\geq 2\right\}\mathbb{1}\left\{Z_{j+1}=0\right\}}_{B_n}  \;.
\end{split}
\end{equation*}

\com{to be checked carefully ...}
We may rewrite $A_n$ and $B_n$ as follows
\begin{align*}
A_n &= M'_n + \sum_{j=1}^n \mathbb{1}\left\{\degree{T_{j+1}}{X_{j}}\geq 2\right\} \Ed_{o, T_0, Z} \left[\Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}= 2\right\}  \middle | \mathcal{G}_{j-1} \right]\;,
\\
B_n &= M_n + \sum_{j=1}^n \mathbb{1}\left\{\degree{T_{j+1}}{X_{j}}\geq 2\right\} \Ed_{o, T_0, Z} \left[\Delta d_j \mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq 3\right\}  \middle | \mathcal{G}_{j-1} \right]\;,
\end{align*}
where, $\mathcal{G}_{j-1}$ is the field generated by  $\mathcal{F}_{j-1}$ and $Z_j$, and $M_n$  is a zero mean martigale (with respect to the filtration $\{\mathcal{G}_{n}\}_{n\geq 0}$) with bounded  increments  
($|M_n-M_{n-1}|\leq 2$, for every $n$). 
The predictable terms satifies  the following bounds \com{check how? all realizations?}
\begin{align*}
\sum_{j=1}^n &\mathbb{1}\left\{Z_{j+1}=1\right\} \mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq 3\right\}\Ed_{o, T_0, Z} \left[\Delta d_j  \middle | \mathcal{G}_{j-1} \right]
\\
&\geq \frac{1}{3} \sum_{j=1}^n \mathbb{1}\left\{Z_{j+1}=1\right\} \mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq 3\right\}
\\
& \geq \frac{1}{3} \sum_{j=1}^n \mathbb{1}\left\{Z_{j+1}=1\right\} \mathbb{1}\left\{Z_{j}=1\right\} \mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}\geq 2\right\}  \;, 
\end{align*}
where, the first inequality follows  by noticing that when $\degree{T_j}{X_{j-1}}\geq 3$ the drift $\Ed_{o, T_0, Z} \left[\Delta d_j  \middle | \mathcal{G}_{j-1} \right]$ is greater  or equal than $1/3$, whereas the last inequality from the fact that $\mathbb{1}\left\{\degree{T_j}{X_{j-1}}\geq 3\right\}\geq \mathbb{1}\left\{Z_{j}=1\right\} \mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}\geq 2\right\}$.  Thus, we  obtain that 
\[
d_n \geq M_n + \frac{1}{3} \sum_{j=1}^n Z_{j+1}\;Z_{j}\; \mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}\geq 2\right\}\;. 
\]

By Azuma's inequality, the process $M_n$ satisfies 
\[
\Pd_{o, T_0, Z} \left(|M_n| > \sqrt{16n\log n}\right)\leq \frac{1}{n^2}\;,
\]
which, in turns, implies that $\Pd_{o, T_0, Z}$-almost surely there exists a $n_0$ such that $M_n \leq \sqrt{16n\log n}$, for all $n\geq n_0$. To control the second term,
\com{ here we should use the previous lemmas....something like...
  choosing  $m$ such that $(m-1)\gamma >2$, we know that $\lim_{n\to \infty}\mathbb{1}\left\{\eta_{\lfloor n/m\rfloor }<n\right\}=1$, $\Pd_{o, T_0, Z}$-almost surely.  
Moreover, by Lemma~\ref{lem:two-sums} and using that $\sum_{k=1}^n p_k p_{k+1} \approx n^{1-2\gamma}$, we obtain that
 for $n$ sufficiently large 
\[
d_n\geq 3 \sqrt{16 n \log n} + c' n^{1-2\gamma} - \sqrt{n \log \log n}\;, \quad 
\text{$\Pd_{o, T_0, Z}$-almost surely}\;.
\] 
Since $\gamma < 1/4$, Equation~\eqref{eq:limsup}  follows. 
}

\end{proof}

\newpage 
\begin{equation*}
\begin{split}
d_n &= \sum_{j=1}^n \Delta d_j = \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}=1\right\} + \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}\geq 2\right\}\;,
\\
&
=\sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}=1\right\}\mathbb{1}\left\{Z_{j}=0\right\} + \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}=1\right\}\mathbb{1}\left\{Z_{j}=1\right\} 
\\
&
\quad +\sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}\geq 2\right\}\mathbb{1}\left\{Z_{j+1}=0\right\} 
\\
& \quad + \underbrace{\sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}= 2\right\}\mathbb{1}\left\{Z_{j+1}=1\right\}}_{\sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}\geq 2\right\}\mathbb{1}\left\{Z_{j+1}=1\right\} + \sum_{j =1}^n \Delta d_j \mathbb{1}\left\{\degree{T_{j-1}}{X_{j-1}}\geq 3\right\}\mathbb{1}\left\{Z_{j+1}=1\right\}}
\end{split}   
\end{equation*}
